Cyclic Arbitrage in Decentralized Exchanges

Decentralized Exchanges (DEXes) enable users to create markets for exchanging any pair of cryptocurrencies. The direct exchange rate of two tokens may not match the cross-exchange rate in the market, and such price discrepancies open up arbitrage possibilities with trading through different cryptocurrencies cyclically. In this paper, we conduct a systematic investigation on cyclic arbitrages in DEXes. We propose a theoretical framework for studying cyclic arbitrage. With our framework, we analyze the profitability conditions and optimal trading strategies of cyclic transactions. We further examine exploitable arbitrage opportunities and the market size of cyclic arbitrages with transaction-level data of Uniswap V2. We find that traders have executed 292,606 cyclic arbitrages over eleven months and exploited more than 138 million USD in revenue. However, the revenue of the most profitable unexploited opportunity is persistently higher than 1 ETH (4,000 USD), which indicates that DEX markets may not be efficient enough. By analyzing how traders implement cyclic arbitrages, we find that traders can utilize smart contracts to issue atomic transactions and the atomic implementations could mitigate users' financial loss in cyclic arbitrage from the price impact.

==> draft-ring.tex <==

\section{Decentralized Exchanges(DEXs)}

Traditional blockchain exchanges were similar to traditional financial markets, such as stocks and brokerage. Transactions are all done through centralized trading platforms, which are owned and operated by a company or an organization that controls over all trades. Cryptocurrency, which is traded on the platform, is stored by a third party. Therefore, users of Centralized Exchanges (CEXs) have faced the risk of losing control of their own assets. CEXs operators may be hacked anytime, resulting in entire funds loss.

Decentralized Exchanges (DEXs) is a solution to protect people's crypto-assets. Users keep coins in their own wallets and use smart contracts and on-chain transactions to realize exchange trading. DEXs operators do not hold customers' funds and just provide automatic matching services for trade orders by public smart contracts hosted on blockchain systems, as well as open-source front-end clients. This ensures decentralized and non-custodial exchange platforms supporting transactions between all coin holders other than registered users.

There are two kinds of DEXs, i.e., order book-based DEXs and liquidity pool-based DEXs. Order book-based DEXs work similarly to CEXs, where users place buy and sell orders at a chosen price. If the price of the sell order is lower than the price of the buy order, the transaction can be completed through DEXs. This mechanism requires high liquidity in order book-based DEXs. Otherwise, users may have to wait for a long time until their transaction orders to be executed. To solve this issue, pool-based DEXs are introduced, where users do not trade with other participants but with liquidity pools, which are smart contracts reserving users' tokens.

In this paper, we focus on liquidity pool-based DEXs. Each liquidity pool contains a pair of coins, and users can buy available tokens from liquidity pools or sell their own tokens to liquidity pools. There are two participants involving in the market, namely liquidity provider and trader. Provider is a trader who provides the trading coin-pair, i.e., the liquidity, to the pool. Providers may also withdraw the coin-pair they reserve in the market. They will be benefited by handling fees incurred with transactions in DEXs because they contribute to the market liquidity. Traders exchange their capital with another available asset in the liquidity pool offered by liquidity providers.

\subsection{Market Liquidity}

\label{sec:liquidity}

Market liquidity is a fundamental feature measuring the ability of investors to trade any number of assets without affecting the price~\cite{chordia2005empirical}. Low market liquidity increases the risk of trades, affects the correct pricing of assets, and thus fosters speculation and market manipulation~\cite{brunnermeier2009market}. The market liquidity of liquidity pool-based DEXs influences price stability and trading activities~\cite{chordia2001market}. Therefore, to stabilize DEXs, it is important to maintain high liquidity and low volatility.

Rather than initiating transactions to put assets into the market and expecting equivalent exchange, liquidity providers just give their money to the liquidity pool. They do not directly profit from this contribution, and the liquidity pool does not return anything back because of this transaction. The liquidity pool will use all the money given by providers to trade with traders, and provides cannot determine the exchange price for each trade. Actually, they have sold their options to the liquidity pool. Therefore, the market mechanism should safeguard the interests of providers in return for their offer of a stable and low-risk market.

\subsection{Automated Market Maker}

Liquidity pools-based DEXs follow a predefined mechanism, i.e., automated market maker(AMM), to indicate the exchange rate of each transaction and the revenue paid to liquidity providers. We denote $X/Y$ as an asset pair of a liquidity pool and $x/y$ as the state of the pool, where $x$ represents the total amount of asset $X$ located in the pool and $y$ the total amount of asset $Y$ available for exchange. Moreover, a liquidity provider $p$ holds a certain amount of liquidity coin, i.e., $c_p$, as proof of the liquidity he contributes to the market. Users can pay liquidity coins to DEXs to withdraw their reserved capital in the smart contract, and these liquidity coins will be destroyed simultaneously. Let us denote $c$ as the entire amount of liquidity coin existing in the market. In this paper, we consider \textbf{constant product AMM}, which occupies 75\% of DEXs market.

A constant product AMM keeps the product $x\times y$ the same before and after each transaction. This product for $X/Y$ will be changed when liquidity providers add or remove the pool's liquidity. Traders leave transaction fees in the liquidity pool for each transaction. These fees will be rewarded to liquidity providers proportional to their contribution when they remove liquidity from the pool. AMM DEXs support three actions as follows:

\begin{itemize}
    \item \textbf{Add liquidity}: A liquidity provider $p$ can reserve $\delta_x$ of its asset $X$ and $\delta_y$ of its asset $Y$ in the liquidity pool, where $\frac{\delta_x}{\delta_y}=\frac{x}{y}$. Then $p$ will earn $\delta_{c_p} = c\cdot\frac{\delta_x}{x}$ liquidity coins for the $X/Y$ asset pair.
    \item \textbf{Remove liquidity}: A liquidity provider $p$ can withdraw $\delta_x$ of $X$ and $\delta_y$ of $Y$ from the $X/Y$ pool with $\delta_{c_p}$ liquidity coins, where $\frac{\delta_x}{x}=\frac{\delta_y}{y}=\frac{\delta_c}{c}$.
    \item \textbf{Exchange asset}: A trader $t$ can exchange $\delta_x$ of asset $X$, with the liquidity pool. He will get $\delta_y$ of asset $Y$ from the pool. The following equation always hold during the transaction: $x\cdot y = (x+\delta_x\cdot r_1)\cdot(y-\frac{\delta_y}{r_2})$, where $r_1$ and $r_2$ denote the transaction fee ratio in asset $X$ and $Y$ respectively. The remaining liquidity in the pool equals to $(x+\delta_x, y-\frac{r_1\cdot r_2\cdot y\cdot\delta_x}{x+r_1\cdot\delta_x})$ In Uniswap, $r_1  = 0.997$ and $r_2=1$, which indicates that the transaction fee is equal to $3$\textperthousand$\cdot \delta_x$.
\end{itemize}

\subsection{Arbitrage in DEXs}

Most DEXs are located on Ethereum, where transactions are transmitted through a peer-to-peer communication protocol. Once the initiator has sent a transaction request, the message will propagate in the network and become available to all participants. Once a profitable transaction is broadcast globally, it will be observed by other arbitrageurs in the network.

However, unlike traditional financial markets, where transactions are executed immediately after user placing orders, DEXs place an order if and only if it has been recorded in a block by miners. The average block generation time is around 15 seconds. Moreover, in more than three-quarters of blocks, transactions within the same block are ordered by the gas price. All these features provide more opportunities for arbitrage bots to manipulate in DEX markets.

The most common arbitrage in DEXs is frontrunning. Because of the information propagation in blockchain networks, arbitrage bots can easily find arbitrage opportunities proposed by other users. The original transaction will not be executed immediately. Therefore, an arbitrageur can submit an identical trading request with a higher gas fee, resulting in a competitive game among arbitrage bots, i.e., a priority gas auction, where miners are served as the auctioneer. These competitions significantly increases the gas price in Ethereum and affect normal trading activities.

Another serious arbitrage in DEXs is the sandwich attack, which is a combination of frontrunning and backrunning. Once an arbitrageur observes a victim transaction submitted by a trader in the network, he will immediately place one order with the same exchange direction just before the victim as the front run and one order with a reversed exchange direction just after the victim as the back run. This attack aims to increase the exchange rate of the victim transaction. Arbitrageur will benefit from the difference between the exchange rate in the front and the back run. This attack also can be realized by a liquidity provider with the same strategy.

In frontrunning and sandwich attacks, arbitrageurs steal the benefits of other traders by placing themselves in advantageous positions in underlying infrastructure. Their behaviors are determined by the latency inherent from on-chain exchanges. In this paper, we focus on another arbitrage which only requires information of transactions validated in blocks. Users do not need to know other's arbitrage orders in advance but just take advantage of the asymmetric market balance across different DEX markets to exploit liquidity providers, which continuously affect the usability of the AMM DEXs.

\subsection{Atomic Transaction}

Ethereum is essentially a replicated state machine. The system state is changed only if the transaction executes successfully. If the transaction fails due to a particular condition it cannot be met, e.g., insufficient transaction fees, conflicting transactions, and prerequisites on market state, the system state will revert to the previous, non-modified state.

Ethereum supports atomic transactions where users can submit several trades executions within a single order. By deploying a proxy contract, if any trade within the same batch fails, the batch will generate an exception of failures, restoring the system state to its pre-execution state. Therefore, the execution of these trades follows an all-or-nothing model, i.e., either all trades are processed sequencially in the market, or none of them affect the liquidity pool, which introduces the atomicity of multiple transactions into AMM DEXs.

\section{Ring Arbitrage in DEXs}

\label{sec:ring}

\subsection{Non-equilibrium of Exchange Rate}

In Uniswap, Curve and many other AMM DEXs, users can exchange between any two currencies if a liquidity pool exists for the currency pair. The exchange rate between the two currencies is determined only by the volume of assets in the liquidity pool, which may differ significantly from the prices in other reference markets. Thus, arbitrageurs can engage in creation-redemption to benefit from the deviated prices of DEXs.

However, these arbitrages need to be deployed in multiple markets simultaneously. The complexity of trading across different markets increases the risk of failure in these strategies. Therefore, arbitrageurs introduce new strategies in a single DEX market. They create a virtual liquidity pool between two cryptocurrencies, i.e., $X/Y$, through intermediary currencies. Then they can earn the exchange rate difference between the original liquidity pool and the virtual liquidity pool of $X$ and $Y$.



\begin{figure*}
    \centering
    \includegraphics[width=16cm]{ex1}
    \caption{Different exchange rate in the ETH/WBTC pool and the virtual pool through LINK in block 11151407.}
    \label{fig:ex}
\end{figure*}



Consider an AMM DEX with three coins, $X$, $Y$, and $Z$. There are three liquidity pools among three coins, i.e., $X/Y$, $Y/Z$, and $Z/X$. We denote $x_1$ and $y_1$ as amount of $X$ and $Y$ in $X/Y$, $y_2$ and $z_2$ as amount of $Y$ and $Z$ in $Y/Z$, and $z_3$ and $x_3$ as amount of $Z$ and $X$ in $Z/X$. Users can directly exchange $\delta_x$ $X$ coins through the $Z/X$ pool and earn $\delta_z$ $Z$ coins, where

\begin{equation}
    \begin{split}
    \delta_z &= r_2\cdot(z_3-\frac{x_3\cdot z_3}{x_3+r_1\cdot\delta_x})\\
    &= \frac{r_1\cdot r_2\cdot z_3\cdot\delta_x}{x_3+r_1\cdot\delta_x}
    \end{split}
    \label{equ:single}
\end{equation}


Or exchange $X$ or $Y$ in $X/Y$ first, and then get $\delta_z'$ $Z$ from the $Y/Z$ pool, where

\begin{equation}
\begin{split}
    \delta_z' &= r_2\cdot(z_2-\frac{y_2\cdot z_2}{y_2+r_1\cdot \frac{r_1\cdot r_2\cdot y_1\cdot\delta_x}{x_1+r_1\cdot\delta_x}})\\
    &= \frac{r_1\cdot r_2\cdot \frac{r_1\cdot r_2\cdot y_1 \cdot z_2}{y_2+r_1\cdot r_2\cdot y_1}\cdot\delta_x}{\frac{x_1 \cdot y_2}{y_2+r_1\cdot r_2\cdot y_1}+r_1\cdot\delta_x}
    \end{split}
    \label{equ:double}
\end{equation}

Compare Equation \ref{equ:single} and \ref{equ:double}, we can observe that the transaction through $X/Y$ and $Y/Z$ is equivalent to an exchange of $\delta_x$ through liquidity pool $X'/Z'$, where $x' = \frac{x_1 \cdot y_2}{y_2+r_1\cdot r_2\cdot y_1}$, and $z'=\frac{r_1\cdot r_2\cdot y_1 \cdot z_2}{y_2+r_1\cdot r_2\cdot y_1}$.

The amount of $Z$ obtained in these two transactions is only determined by $X/Z$ and $X'/Z'$, respectively. The market parameters in these three pools are independent. Therefore, we can obtain different exchange rates between the two coins in the same market. Even rational traders are incentivized to balance the market price across different pools. The complex trading environment and the incomplete real-time market information influence traders' behaviors and drive the DEX market to stay in a non-equilibrium state.

Therefore, with intermediary coin $Y$, we can construct a virtual liquidity pool between $X$ and $Z$ with a different exchange rate. We take the liquidity pool of Ethereum, ChainLink, and Wrapped Bitcoin in block 11151407 as an example, which is shown in Figure \ref{fig:ex}. We can either directly trade 0.005 ETH for 0.0001466 WBTC through the ETH/WBTC pool, or exchange 0.1694 LINK first from the ETH/LINK pool and then obtain 0.0001496 WBTC through the LINK/WBTC pool.

\subsection{Arbitrage Ring Transactions}

As we discussed above, users can build a virtual liquidity pool between $X$ and $Z$. Follow this idea, and we may consider $Z$ as an intermediary to build a virtual liquidity pool between $X$ and $X$ by trading along the path $X\rightarrow Y\rightarrow Z\rightarrow X$. The amount of $X$ user earns from these transactions, i.e., $\delta_x'$, can be represented as,

\begin{equation}
    \delta_x' = \frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot y_1\cdot z_2\cdot x_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2} \cdot\delta_x}{\frac{x_1\cdot y_2\cdot z_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2}+r_1\cdot\delta_x}
\end{equation}

These cross-pool transactions can be equated to a single exchange with $\delta_x$ in $X/X'$ pool, where $x = \frac{x_1\cdot y_2\cdot z_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2}$, $x' = \frac{r_1^2\cdot r_2^2 \cdot y_1\cdot z_2\cdot x_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2}$.
If the exchange rate of the $X/X'$ pool is larger than 1, i.e., $\delta_x' > \delta_x$, arbitrageurs will directly earn money from the virtual liquidity pool without any additional operation. The trading path of these ring transactions is not limited with three coins. Arbitrageurs might 

Figure \ref{fig:ring} shows a ring transaction in Ethereum, executed on October 30th, 2020. A ring transaction is a batch of atomic trades deplyed by a smart contract proxy. These trades are executed if and only if the outcome of these sequential exchanges is larger than the trades' input. In this ring transaction, the arbitrageur traded 285.71 USDC in Uniswap V2 through four different liquidity pools across USD Coin, Tether USD, Seal Finance, Keep3rV1, and finally get 303.68 USDC from the KP3R/USDC pool. The arbitrageur earned 17.97 dollars from this transaction.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{ex2}
    \caption{Example ring transaction observed in Ethereum.}
    \label{fig:ring}
\end{figure}

%\subsection{Attacks to Liquidity Provider}

%In Section \ref{sec:liquidity}, we discussed the importance of liquidity of DEXs and how liquidity providers promote market stability. The only profit of being a liquidity provider for DEXs is from charging the handling fee for each transaction.

%尽管套利行为在当前市场上，套利行为被认为是有利于金融市场的流动性,促进市场资源逐渐走向平衡,然后对市场资源进行整合。

%Traders can control their trades more actively in DEXs because they can determine the trading direction, trading amount, slippage tolerance, and transaction deadline of each transaction by themselves. However, liquidity providers can only deposit or withdraw the asset pair in the pool and wait for uncertain outcomes, which leaves space for traders to attack them without risk.

Unlike front-running~\cite{daian2020flash} and sandwich attacks~\cite{zhou2020high}, where victims are traders, ring transactions does not hurt the benefit of any participant. On the contrary, it balances the price across several markets. In Figure \ref{fig:pool}, we present the change in the liquidity pool caused by the ring arbitrage transaction. the product of transaction rates of USDC/USDT, USDT/SEAL, SEAL/KP3R, and KP3R/USDC is 0.89 before the ring transaction, while the product moves to 0.97 after the arbitrage's action.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{ex3}
    \caption{Liquidity in market pool before and after transaction 0xcf709…}
    \label{fig:pool}
\end{figure}

The ring transaction is an arbitrage in liquidity pool-based DEXs because it takes advantage of the price difference cross several markets. Ring arbitrages cause price convergence between pools where traders may sell or buy coins with the same price in different markets. After the ring arbitrage shown in Figure \ref{fig:ring}, the exchange ratio between any pair of coins are closer. Therefore, arbitrageurs can easily balance the market with the atomic ring transaction, which indicated the market efficient of liquidity pool-based DEXs is high~\cite{damghani2013non}.

%We answer this question by studying the market liquidity before and after the ring arbitrage transaction.  For USDT, SEAL, and KP3R, assets were just moved from one pool to another. At the same time, the sum of each asset in the market did not change. However, for USDC, the original reserve in USDC/USDT and KP3R/USDC pools is 7221682, whereas the rest of USDC in these two pools is only 7221664. The arbitrageur did not only take 18 USDC from the market but also hurt the market liquidity because he has not brought any new coins to the market. The liquidity provider could only withdraw fewer assets from the market with the same amount of liquidity coins. Therefore, the profit of ring arbitrages comes from attacks on liquidity providers.
\label{sec:balance}
\section{Impact on Participants}

In this section, we consider how ring arbitrages influence other participants' profit, i.e., liquidity providers and traders. We argue that ring transactions benefit liquidity providers because they make the market go through more trades before reaching equilibrium. Corresponding to this, the profit of traders will decrease while they still have chance to arbitrage in the market. To illustrate the impact of ring arbitrages on participants' profit, we consider a simple model with three coins $X$, $Y$, and $Z$.

\subsection{Profit Analysis in Closed Markets}

First, let's consider transactions inside the market with coin $X$, $Y$, and $Z$. We have presented a ring transaction which can balance the market price cross several pools in DEXs in Section \ref{sec:balance}. If, after the ring arbitrage, there is no space for traders to profit themselves with the price difference, we can conclude that the ring arbitrageur exhausts all the market benefits, which is denoted as $b_M$. This atomic ring transaction can be considered several single arbitrages that balance the market with the minimum costs. Therefore, liquidity providers earn a minimal possible transaction fee for any transactions balancing the market, and other traders get nothing from the market. Then we discuss two other observations in the closed market,

\begin{proposition}
    If ring arbitrages are not possible in the market, then others arbitrageurs can not benefit by single trades pair.
    \label{propo:im1}
\end{proposition}

\begin{proof}
We prove this by contradiction. We assume there is a beneficial single trades pair in a non-ring arbitrage market, i.e., buying $Z$ from the pool $Z/X$ with a lower price in the unit of $X$ and selling $Z$ from the pool $X/Y, Y/Z$ with a higher price in the unit of $X$.

Therefore, we can have,

$$\frac{\frac{r_1\cdot r_2\cdot z_3\cdot\delta_x}{x_3+r_1\cdot\delta_x}}{\delta_x}<\frac{\frac{\delta_x\cdot \frac{z_2\cdot y_1}{y_1+r_1\cdot r_2\cdot y_2}}{\frac{r_1^2\cdot r_2^2\cdot y_2\cdot x_1}{y_1+r_1\cdot r_2\cdot y_2}-\delta_x\cdot r_1}}{\delta_x}
$$

Let $\delta_z = \frac{\delta_x\cdot \frac{z_2\cdot y_1}{y_1+r_1\cdot r_2\cdot y_2}}{\frac{r_1^2\cdot r_2^2\cdot y_2\cdot x_1}{y_1+r_1\cdot r_2\cdot y_2}-\delta_x\cdot r_1}$, we can conclude that 

$$\delta_z< \frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot y_2\cdot x_1\cdot z_3}{y_1\cdot x_3+r_1\cdot r_2\cdot y_2\cdot x_3+r_1^2\cdot r_2^2\cdot y_2\cdot x_1} \cdot\delta_z}{\frac{z_2\cdot y_1\cdot x_3}{y_1\cdot x_3+r_1\cdot r_2\cdot y_2\cdot x_3+r_1^2\cdot r_2^2\cdot y_2\cdot x_1}+r_1\cdot\delta_z}$$

There is a ring arbitrage opportunity through $Z/Y\rightarrow Y/X\rightarrow X/Z$, which contradicts to our assumption.

\end{proof}


\begin{proposition}
    If after the ring arbitrage the market is not balanced, then the profit of following single trades is smaller than $b_M$, and the profit of liquidity providers is higher than the minimum possible transaction fee.
    \label{propo:im2}
\end{proposition}


\begin{proof}

Take market $X/Y$ as an example. Fist, consider the scenario where the market is balance by the ring transaction. The product of the volume of $X$ and $Y$ before the ring transaction is $x_1\cdot y_1$ and the product moves to $P=x_1\cdot y_1+(1-r_1)\delta_x\cdot (y-\delta_y)+(\frac{1}{r_2}-1)\cdot \delta_y\cdot (x+\delta_x)>x_1\cdot y_1$ because $r_1, r_2<1$. We denote the ratio between liquidity of $X$ and $Y$ as $k$.

In the second scenario, we need a single additional transaction moving the ratio between $X$ and $Y$ to $k$ and the product of the volume, i.e., $p'$, is larger than $P$. Therefore, liquidity providers can share more assets compared to the first scenario. And the profit caused by the unbalanced price is share by the ring arbitrageur and others. Thus, none of them is larger than $b_M$.
\end{proof}

\subsection{Profit Analysis in Open Markets}

Arbitrageurs are not limited to trading in AMM DEXs, while cryptomoney prices are also influenced by participants of other markets, e.g., CEXs. Therefore, in this section, we consider how traders behave when there exist external markets.

Let us assume we have three coins $X$, $Y$, and $Z$ in the market. Initially, prices of $X$, $Y$, and $Z$ in external markets are $p_x$, $p_y$, and $p_z$, respectively. After several arbitrage tradings, prices of $X$, $Y$, and $Z$ converges to $p_x'$, $p_y'$, and $p_z'$~\cite{angeris2020improved}, while the volume of coins in each pool is $x_1/y_1$, $y_2/z_2$, and $z_3/x_3$.

Consider a series of transactions which are executed by rational traders without ring transactions and denote transactions happen in the AMM DEX market as $t_1, t_2, \ldots, t_n$. We analyze how ring transactions change the arbitrageurs' profit. Let's assume there is a ring transaction $t_r$ happens after $t_i$, then there are two possible scenarios after the execution of $t_r$.

In the first case, the amount of coins in each pool is exactly $x_1/y_1$, $y_2/z_2$, and $z_3/x_3$, then we conclude that transaction $t_{i+1}$, $t_{i+2}$, and $t_{i+3}$ are equal to $t_r$, because traders are rational and use optimal strategies to arbitrage. Therefore, the ring transaction does not change the profit of any participate in the market while the ring arbitrage takes all benefits from issuer of $t_{i+1}$, $t_{i+2}$, and $t_{i+3}$.

In the second case, we argue that traders will pay more transaction fees to the liquidity providers. Take the pool $X/Y$ as an example. Assume that the amount of coins in the pool before $t_r$ is $x_b/y_b$, and it moves to $x_a/y_a$, while $\frac{x_a}{y_a}\neq\frac{x_1}{y_1}$, which means there is still space for arbitrage in the AMM DEXs. Then, there will be a rational trader exchange $A$ and $B$ in the pool to drive the price to $x_1/y_1$. Then we compare two trading behavior, i.e., if there is no ring arbitrage, the pool liquidity moves from $x_b/y_b$ to $x_1/y_1$ by a transaction $t_{i+1}$, and if there exists $t_r$, the pool liquidity moves from $x_b/y_b$ to $x_a/y_a$ by $t_r$, and finally reaches $x'/y'$ where  $\frac{x'}{y'}=\frac{x_1}{y_1}$ by a transaction $t'$.

We assume $t_{i+1}=(+\delta_{x}^{i+1}, -\delta_y^{i+1})$. The trades of $X/Y$ within $t_r$, i.e., $t_{r1}$ and $t'$ can happen in three scenarios according to the market balance in AMM DEXs.

\begin{itemize}
    \item $t_{r1}=(+\delta_{x}^{r1}, -\delta_y^{r1})$ and $t'=(-\delta_x', +\delta_y')$: 
    We can deduct that $\delta_x^{r1}>\delta_{x}^{i+1}$. It turns out that $t_r$ leaves $\delta_x^{r1}\cdot(1-r_1)$ and $x_a\cdot y_a>x_1\cdot y_1$. Therefore, more transaction fees are remained in the liquidity pool because of the ring transaction.
    
    \item $t_{r1}=(-\delta_{x}^{r1}, +\delta_y^{r1})$ and $t'=(+\delta_x', -\delta_y')$: 
    We can deduct that $\delta_x'>\delta_{x}^{i+1}$. It turns out that $t'$ leaves $\delta_x'\cdot(1-r_1)$ and $x'\cdot y'>x_1\cdot y_1$. Therefore, more transaction fees are remained in the liquidity pool because of the ring transaction.
    
    \item $t_{r1}=(+\delta_{x}^{r1}, -\delta_y^{r1})$ and $t'=(+\delta_x', -\delta_y')$:
    If the ring transaction 
\end{itemize}



\section{Dynamic Transaction Fee}

Liquidity providers benefit in DEXs by charging trades fees from traders in each transaction. For example, before and after a transaction in Uniswap, the product of the number of two assets in the pool does not keep the same. Even though the market does not charge extra handling fees from the output of transactions, only $r_1\cdot\delta_x$ of $X$ is counted as a effective trading input to the Uniswap, resulting in the product not being a constant. The fixed amount of the input, i.e., 3\textperthousand of $\delta_x$, will be deducted from the transaction and remain in the liquidity pool. Liquidity providers will share the commission proportional to the liquidity coin they have when withdrawing reserve currency from the pool. The higher the transaction fee, the more providers get out of each transaction.

Transaction fees not only allow liquidity providers to benefit from each successful trade request in response to their contribution to the system. It also protects the liquidity provider from ring attacks. Since the revenue of ring attacks is deduced by the handling fee after each transaction, arbitrageurs will not apply the ring attack if the there is no space for arbitrage. Therefore, the transaction fee determines how heavily arbitrageurs will hurt the liquidity of markets.

In this section, we study the influence of transaction fees on ring attacks in AMM DEXs. We first analyze the arbitrage model of ring attacks and indicate how transaction fees affect the attack efficiency theoretically. Then, we propose a dynamic transaction fee solution to defend the existing attacks in the market. We evaluate this mechanism's performance on historical data, i.e., how much will it prevent existing ring attacks and how much it will interfere with normal transactions.



\subsection{Arbitrage Model}

We follow the same setting as described in Section \ref{sec:ring}, starting with the market with three coins $X$, $Y$, and $Z$. Without loss of generality, we assume that an arbitrageur $A$ who keeps $\delta_x$ of $X$ would like to apply a ring attack to earn more $X$ from the market. $A$ has two possible trading strategies, namely exchanging $\delta_x$ through $X\rightarrow Y\rightarrow Z\rightarrow X$ path or $X\rightarrow Z\rightarrow Y\rightarrow X$ path. We denote $U_{XYZX}$ and $U_{XZYX}$ as the utility of these two strategies respectively, where,

\begin{equation}
    \begin{split}
    U_{XYZX} &= \delta_x' - \delta_x\\
    &=(\frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot y_1\cdot z_2\cdot x_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2}}{\frac{x_1\cdot y_2\cdot z_3}{y_2\cdot z_3+r_1\cdot r_2\cdot y_1\cdot z_3+r_1^2\cdot r_2^2\cdot y_1\cdot z_2}+r_1\cdot\delta_x}-1)\cdot \delta_x
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
    U_{XZYX} &= \delta_x' - \delta_x\\
    &=(\frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot z_3\cdot y_2\cdot x_1}{z_2\cdot y_1+r_1\cdot r_2\cdot z_3\cdot y_1+r_1^2\cdot r_2^2\cdot z_3\cdot y_2}}{\frac{x_3\cdot z_2\cdot y_1}{z_2\cdot y_1+r_1\cdot r_2\cdot z_3\cdot y_1+r_1^2\cdot r_2^2\cdot z_3\cdot y_2}+r_1\cdot\delta_x}-1)\cdot \delta_x
    \end{split}
\end{equation}

\begin{proposition}
For each trading cycle, the arbitrageur can benefit from trading in at most one direction.
\label{pro:1}
\end{proposition}

\begin{proof}
When $\delta_x = 0$, both $U_{XYZX}$ and $U_{XZYX}$ have value 0. Then we consider the first derivative of the utility function of the variable $\delta_x$. 

Take $U_{XYZX}$ as an example, the first derivative of the function at $\delta_x = 0$ equals to,

\begin{equation}
    \frac{\partial U_{XYZX}}{\partial \delta_x}\bigg|_{\delta_x = 0}=\frac{r_{1}^3\cdot r_{2}^3\cdot x_{3}\cdot y_{1}\cdot z_{2}}{x_{1}\cdot y_{2}\cdot z_{3}} -1
\end{equation}

Symmetrically, we obtain the first derivative of $U_{XZYX}$ at $\delta_x = 0$ as,

\begin{equation}
    \frac{\partial U_{XZYX}}{\partial \delta_x}\bigg|_{\delta_x = 0}=\frac{r_{1}^3\cdot r_{2}^3\cdot x_{1}\cdot y_{2}\cdot z_{3}}{x_{3}\cdot y_{1}\cdot z_{2}} -1
\end{equation}

Because $r_1,r_2\leq 1$, one of these two derivatives at $\delta_x = 0$ must be small or equal to 0, w.l.o.g, we assume $\frac{\partial U_{XYZX}}{\partial \delta_x}\leq 0$

By computing the second derivative of $U_{XYZX}$, we know that $\frac{\partial^2 }{\partial \delta_x^2}U_{XYZX}$ is negative for all $\delta_x\in R^+$. Therefore, $U_{XYZX}$ is a monotone decreasing function in its domain, and the maximum value of $U_{XYZX}$ is 0 at $\delta_x=0$. The arbitrageur cannot benefit from trading $\delta_x$ through $X/Y$, $Y/Z$, and $Z/X$ pools, sequentially.

\end{proof}
%我们发现这个收益和transaction fee有很大的关系，如果费用越高，那么收益就越少。如果费用是0的话，那么无论如何都可以从市场中获利，伤害到了provider的利益，所以我们认为手续费是保护提供者的一个重要因素
From Proposition \ref{pro:1}

\begin{proposition}
If there is no transaction fee in the market, i.e., $r_1=1$ and $r_2=1$, then the arbitrageur can always benefit from the market by a ring strategy unless the market is balance.
\label{pro:2}
\end{proposition}

\begin{proof}

Based on the computation result in the proof of \ref{pro:1}, we can derive the the first derivative of $U_{XYZX}$ and $U_{XZYX}$ at $\delta_x = 0$, where $r_1=1$ and $r_2=1$,

\begin{equation}
    \frac{\partial U_{XYZX}}{\partial \delta_x}\bigg|_{\delta_x = 0}=\frac{x_{3}\cdot y_{1}\cdot z_{2}}{x_{1}\cdot y_{2}\cdot z_{3}} -1
\end{equation}

and,

\begin{equation}
    \frac{\partial U_{XZYX}}{\partial \delta_x}\bigg|_{\delta_x = 0}=\frac{x_{1}\cdot y_{2}\cdot z_{3}}{x_{3}\cdot y_{1}\cdot z_{2}} -1
\end{equation}.

If the market is not balance, i.e., $\frac{x_1}{y_1}\cdot\frac{y_2}{z_2}\cdot\frac{z_3}{x_3}\neq 1$, then either one of $\frac{x_{3}\cdot y_{1}\cdot z_{2}}{x_{1}\cdot y_{2}\cdot z_{3}}$ and $\frac{x_{1}\cdot y_{2}\cdot z_{3}}{x_{3}\cdot y_{1}\cdot z_{2}}$ is strictly larger than 1. 

W.l.o.g, we assume that $\frac{x_{3}\cdot y_{1}\cdot z_{2}}{x_{1}\cdot y_{2}\cdot z_{3}}>1$. The first derivative of $U_{XYZX}$ is larger than 0 at $\delta_x=0$ and $U_{XYZX}=0\bigg|_{\delta_x = 0}$. Therefore, there exists a value $\Delta>0$ such that $U_{XYZX}(\delta_x>0)$ where $\delta_x=\Delta$. The arbitrageur can benefit from a ring transaction with $\Delta$ of $X$ through $X\rightarrow Y\rightarrow Z\rightarrow X$ path.

\end{proof}

\subsection{Dynamic Transaction Fee}

\begin{lemma}
For a ring transaction through a path with $n+1$ edges $X\rightarrow Y^1\rightarrow Y^2\rightarrow \ldots \rightarrow Y^n\rightarrow X$, the first deviation of the utility function at $\delta_x=0$ is $\frac{\partial U}{\partial \delta_x}\bigg|_{\delta_x = 0}=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot x_{n+1}\cdot y^1_1\cdot y^2_2\cdot \ldots\cdot y^n_n}{x_1\cdot y^1_2\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}$.
\label{lemma:1}
\end{lemma}

\begin{proof}
We prove this lemma by induction. We has already shown it is correct in the proof of Proposition \ref{pro:1} when $n=2$.

As we discussed in Section \ref{sec:ring}, if we exchange $\delta_x$ through $X/Y^1$ pool to get $\delta_y^1$, and obtain $\delta_y^2$ from $Y^1/Y^2$ by trading $\delta_y^1$ right after, these two atomic transactions can is equivalent to a single transaction with $\delta_x$ in a virtual pool $X_v/Y_v$, where $x_v = \frac{x_1 \cdot y^1_2}{y^1_2+r_1\cdot r_2\cdot y^1_1}$, and $y_v=\frac{r_1\cdot r_2\cdot y^1_1 \cdot y^2_2}{y^1_2+r_1\cdot r_2\cdot y^1_1}$.

We assume that the statement is correct for any $n$-path ring transaction. Consider a ring transaction through a $n+1$-path $X\rightarrow Y^1\rightarrow Y^2\rightarrow \ldots \rightarrow Y^n\rightarrow X$, which is equivalent to a $n$-path ring transaction through $X_v\rightarrow Y_v\rightarrow \ldots \rightarrow Y^n\rightarrow X$, where the first deviation of the utility function at $\delta_x=0$ is,

\begin{equation}
    \begin{split}
        \frac{\partial U}{\partial \delta_x}\bigg|_{\delta_x = 0}&=\frac{r_1^{n}\cdot r_2^{n}\cdot x_{n+1}\cdot y_v\cdot \ldots\cdot y^n_n}{x_v\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}\\
        &=\frac{r_1^{n}\cdot r_2^{n}\cdot x_{n+1}\cdot \frac{r_1\cdot r_2\cdot y^1_1 \cdot y^2_2}{y^1_2+r_1\cdot r_2\cdot y^1_1}\cdot \ldots\cdot y^n_n}{\frac{x_1 \cdot y^1_2}{y^1_2+r_1\cdot r_2\cdot y^1_1}\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}\\
        &=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot x_{n+1}\cdot y^1_1\cdot y^2_2\cdot \ldots\cdot y^n_n}{x_1\cdot y^1_2\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}
    \end{split}
\end{equation}

Therefore, the statement in Lemma \ref{lemma:1} also hold for any $n+1$ ring transaction.

\end{proof}

\begin{proposition}
There exist a threshold $t$ such that there does not exist any ring arbitrage in the market if the transaction rate $r_1\cdot r_2 \leq t$.
\end{proposition}

\begin{proof}

Consider a ring trading path with length $n+1$ $X\rightarrow Y^1\rightarrow Y^2\rightarrow \ldots \rightarrow Y^n\rightarrow X$ and its reversed path $X\rightarrow Y^n\rightarrow Y^{n-1}\rightarrow \ldots \rightarrow Y^1\rightarrow X$. According to Proposition \ref{pro:2}, if there is no transaction fee, then the arbitrageur can benefit from one of them, w.l.o.g, we assume the beneficial one is the first path.

This implies that the first derivative of the utility function at $\delta_x=0$ is larger than 0 when $r_1=r_2=0$. Therefore, we can derive the following inequality such that $\frac{x_{n+1}\cdot y^1_1\cdot y^2_2\cdot \ldots\cdot y^n_n}{x_1\cdot y^1_2\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}>1$.

However, if $r_1\cdot r_2 \leq r = \sqrt[n+1]{\frac{x_{n+1}\cdot y^1_1\cdot y^2_2\cdot \ldots\cdot y^n_n}{x_1\cdot y^1_2\cdot y^2_3\cdot\ldots\cdot y^n_{n+1}}}$, the arbitrageur cannot profit from $X\rightarrow Y^1\rightarrow Y^2\rightarrow \ldots \rightarrow Y^n\rightarrow X$ anymore.

For each ring path in the market, we can compute a threshold $r$ and assign $t$ to the minimum value among all thresholds. Then the arbitrageur cannot benefit from the market by applying a ring trading strategy.

\end{proof}

%r2*(x3-(x3*z3)/(z3+r1*r2*(z2-y2*z2/(y2+r1*r2*(y1-x1*y1/(x1+r1*x))))))-x

%$\frac{\partial f}{\partial x} = -{{\left(\left(x_{1}^2+2\cdot x\cdot x_{1}+x^2\right)\cdot y_{2}^2+\left(2\cdot x\cdot  x_{1}+2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+x^2\cdot y_{1}^2\right)\cdot z_{3}^2+ \left(\left(-x_{1}\cdot x_{3}+2\cdot x\cdot x_{1}+2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+2 \cdot x^2\cdot y_{1}^2\right)\cdot z_{2}\cdot z_{3}+x^2\cdot y_{1}^2\cdot z_{2}^2}\over{ \left(\left(x_{1}^2+2\cdot x\cdot x_{1}+x^2\right)\cdot y_{2}^2+\left(2\cdot x\cdot  x_{1}+2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+x^2\cdot y_{1}^2\right)\cdot z_{3}^2+ \left(\left(2\cdot x\cdot x_{1}+2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+2\cdot x^2\cdot y_{1}^2 \right)\cdot z_{2}\cdot z_{3}+x^2\cdot y_{1}^2\cdot z_{2}^2}}$

%$\frac{\partial f}{\partial x} = -{{\left(\left(x_{1}^2+2\cdot r_{1}\cdot x\cdot x_{1}+r_{1}^2\cdot x^2\right)\cdot  y_{2}^2+\left(2\cdot r_{1}^2\cdot r_{2}\cdot x\cdot x_{1}+2\cdot r_{1}^3\cdot r_{2}\cdot x^2 \right)\cdot y_{1}\cdot y_{2}+r_{1}^4\cdot r_{2}^2\cdot x^2\cdot y_{1}^2\right)\cdot z_{3}^2 +\left(\left(-r_{1}^3\cdot r_{2}^3\cdot x_{1}\cdot x_{3}+2\cdot r_{1}^3\cdot r_{2}^2\cdot x \cdot x_{1}+2\cdot r_{1}^4\cdot r_{2}^2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+2\cdot r_{1}^5\cdot  r_{2}^3\cdot x^2\cdot y_{1}^2\right)\cdot z_{2}\cdot z_{3}+r_{1}^6\cdot r_{2}^4\cdot x^2\cdot  y_{1}^2\cdot z_{2}^2}\over{\left(\left(x_{1}^2+2\cdot r_{1}\cdot x\cdot x_{1}+r_{1}^ 2\cdot x^2\right)\cdot y_{2}^2+\left(2\cdot r_{1}^2\cdot r_{2}\cdot x\cdot x_{1}+2\cdot r_{1}^3 \cdot r_{2}\cdot x^2\right)\cdot y_{1}\cdot y_{2}+r_{1}^4\cdot r_{2}^2\cdot x^2\cdot y_{1}^2 \right)\cdot z_{3}^2+\left(\left(2\cdot r_{1}^3\cdot r_{2}^2\cdot x\cdot x_{1}+2\cdot r_{1}^ 4\cdot r_{2}^2\cdot x^2\right)\cdot y_{1}\cdot y_{2}+2\cdot r_{1}^5\cdot r_{2}^3\cdot x^2\cdot y_{1} ^2\right)\cdot z_{2}\cdot z_{3}+r_{1}^6\cdot r_{2}^4\cdot x^2\cdot y_{1}^2\cdot z_{2}^2}}$

%${{x_{3}\cdot y_{1}\cdot z_{2}}\over{x_{1}\cdot y_{2}\cdot z_{3}}}-1$



==> draft.tex <==

\begin{figure*}

\begin{minipage}[t]{0.245\linewidth}
\centering
\setcaptionwidth{0.9\linewidth}
\includegraphics[width=3cm]{start_token_counts.png}
\caption{The starting token as cyclic arbitrages.}
\label{fig:starttoken}
\end{minipage}
\begin{minipage}[t]{0.245\linewidth}
\centering
\setcaptionwidth{0.9\linewidth}
    \input{daily_txs}
    \caption{Daily number of cyclic arbitrages.}
    \label{fig:num}
\end{minipage}
\begin{minipage}[t]{0.245\linewidth}
\centering
\setcaptionwidth{0.9\linewidth}
\includegraphics[width=3cm]{start_token_counts.png}
\caption{The starting token as cyclic arbitrages.}
\label{fig:starttoken}
\end{minipage}
\begin{minipage}[t]{0.245\linewidth}
\centering
\setcaptionwidth{0.9\linewidth}
    \input{daily_txs}
    \caption{Daily number of cyclic arbitrages.}
    \label{fig:num}
\end{minipage}

\end{figure*}


\section{Introduction}

Decentralized Exchanges (DEXs) of cryptocurrencies have attracted a lot of attention since their emergence. Compared to traditional centralized exchanges (CEXs), where transactions are all done through centralized trading platforms, which are owned and operated by a company or an organization that controls all trade, DEXs ensure decentralized and non-custodial exchanges. Users swap assets on DEXs by interacting with the DEXs smart contracts through on-chain transactions, while no third party is involved throughout the whole process.

In May 2020, Uniswap V2 was officially launched on Ethereum~\cite{uni2la}, which is one of the most prominent examples of DEXs. As of November 2020, it has amassed total market liquidity of over 3 billion USD and attracted a trading volume of over 400 million USD per day. Uniswap is an Automated Market Maker (AMM) DEX. As opposed to other DEXs, which execute limit order books (LOB) following deterministic nature, AMM DEXs have introduced algorithmic mechanisms to perform market making, i.e., enabling the purchase and sale of assets and setting prices for each trade automatically. 

In AMM DEXs, the exchange rate of each trade is determined by predefined algorithms according to the market liquidity reserves, which is public information to everyone due to the transparent nature of blockchain. Therefore, arbitrageurs can prejudge the price of each upcoming transaction in advance and exploit the price difference to their advantage across different markets~\cite{makarov2020trading}. Past work has acknowledged arbitrageur behavior based on front-running~\cite{daian2020flash}. Unfortunately, these arbitrages bring threats to the market and system stability. Arbitrageurs optimize network latency aggressively and conduct priority gas auctions to front-run profitable trades~\cite{lewis2014flash}, which results in excessive transaction fees affecting normal users in blockchain ecosystems. Moreover, because of the high miner-extractable value, fee-based forking attacks and time-bandit attacks are created and bring systemic consensus-layer vulnerabilities~\cite{daian2020flash}. Other work has considered arbitrages that take advantage of loopholes in DEXs market mechanism to reap benefits maliciously, including a combination of front- and back-running~\cite{zhou2020high}, and price oracle manipulations~\cite{qin2020attacking}. These arbitrages attack a certain trader and profit themselves by harming the target victim.

In this paper, we study a new arbitrage behavior, i.e., cyclic arbitrage, observed in Uniswap V2. While Uniswap V1 only allowed trading from/to ETH, V2 allows users to create trading pools between any pair of tokens, without the need for ETH as an intermediary currency~\cite{uni2}. Each pool then allows for automatic trading between a pair of tokens. Assume we have three currencies $A, B, C$, and three liquidity pools between any two pairs: $A\rightleftharpoons B, B\rightleftharpoons C$ and $C\rightleftharpoons A$. Each of these pools has an exchange rate, which changes over time, depending on the recent trades in that pool. Given these three pools, arbitrageurs are now able to trade currencies cyclically: A trader can trade currency $A$ for $B$ in $A\rightleftharpoons B$, then $B$ for $C$ in $B\rightleftharpoons C$, and finally $C$ for $A$ in $C\rightleftharpoons A$ again, to benefit themselves from the differences of exchange rates.

As of November 2020, there are over 20,000 trading pairs on Uniswap, enables 870 cyclic arbitrages per day for a total daily income of 149.79 ETH on average. To better understand this emerging financial behavior in AMM DEXs, we conduct a mixed-method study, including theoretical analysis and empirical evaluation, on cyclic arbitrages. We first formalize a theoretical model of AMM DEX with multiple liquidity pools and the cyclic arbitrage in constant product AMM, i.e., Uniswap. We study the market conditions when cyclic arbitrage opportunities exist. We find that the amount of potential cyclic arbitrages decreases as the transaction fee rises. If the product of the exchange rate along the trading path is greater than the product of the transaction rate, then arbitrageurs can make a profit with these cyclic transactions. 

We further analyze the impact of cyclic arbitrages on the market and participants. Previous studies~\cite{qin2020attacking, zhou2020high, daian2020flash} focused on the negative impact of arbitrages to the market and the blockchain system. However, we find that cyclic arbitrages balance the exchnge rates across the market, improving the overall market efficiency, which is good for traders (who trade in a fair market), and as a consequence also for the liquidity providers (since these arbitrages also increase the number of trades, and as such their income from fees). Since cyclic arbitrageurs can deploy atomic transactions to guarantee their income, it is a win for everybody involved.

Beyond theoretical analysis, we quantitatively study trading information on Uniswap from May 2020 to November 2020.

To test this hypothesis 0. cycle length vs. amount 1. CA vs. market balance 2. CA vs. liquidity 3. CA vs. normal transactions 4. CAff vs. Annualized Interest Rate?-not sure

Understanding failures of cyclic transactions , why loose money, successful rate, profit vs revenue

More insight, transaction fee vs cycles, which market dominate prices

This paper makes the following contributions:

\section{Background}

\subsection{Ethereum}

Ethereum is a public blockchain platform, which supports Turing complete smart contract functions. Compared to earlier blockchain systems, such as Bitcoin, Ethereum is not only implementing a decentralized cash system that allows peer-to-peer transactions but also ``the world computer''. Smart contracts are ``software'' running on this ``computer''. Ethereum deploys a decentralized virtual machine, i.e., Ethereum Virtual Machine (EVM), to execute smart contract code.

There are two kinds of accounts in Etheurem, namely externally owned accounts (EOAs), i.e., those controlled by human users with the corresponding private key, and smart contract accounts (CAs), controlled by executable code developed by human users~\cite{wood2014ethereum}. Each account has a fixed address, which serves as the identity of the account in the Ethereum system. Meanwhile, the system also keeps an account state for each participant. The state of an EOA is the current balance of ETH in the account, while the state of a smart contract account is the current data stored in its variables. States of accounts are stored in an independent key-value database, i.e., stateDB.

An Ethereum transaction is broadcast by an EOA user to the Ethereum network. 
EOAs can send three types of transactions: \textbf{simple transaction}, of which recipient is another address (account) to transfer the native currency, Ether; \textbf{smart contract creation transaction}, of which recipient is the null address to create a new smart contract; \textbf{smart contract execution transaction}, of which recipient is a smart contract address to execute a specific function of that contract.
When a transaction is recorded in the block, the operation corresponding to the message takes effect. The miner who creates the block modifies the state of corresponding accounts based on the messages. Each step of the miner's operation consumes a certain amount of gas, and the amount of gas consumed in each block is capped. Users need to specify a gas price for the operation execution when sending transactions. The fee paid by the initiator to miners for each transaction is determined by the amount of gas consumed and the gas price, i.e., transaction fee=gas price$\times$consumed gas.

After the transaction is executed, a transaction receipt will be generated and included in Ethereum blocks. The receipt includes the information on whether the transaction has been executed successfully, the transaction cost, the identity of the transaction and the block, and other information generated during the execution of the transaction.

\subsection{Smart Contract and ERC-20 Token Standard}

A smart contract is a set of executable programs, which are written in high-level languages, e.g., Solidity. Creators compile them into bytecode and send them within a message to the \textit{null} address, declaring the creation of a smart contract and the address of the contract will be determined by the sender's address and the message nonce. The creation message of a smart contract can be either sent by an EOA or a smart contract address. After the contract creation, all addresses can send messages to this address to invoke functions implemented by the contract. EVM will execute the function and update the smart contract state.

Based on the support of the smart contract, users can deploy cryptocurrency (token) other than Ether on Ethereum infrastructure. These smart contracts have to follow some rules, and the most widely used one of them is the ERC20 standard, which requires an \textit{approve()} function and a \textit{transferFrom()} function. When the address $A$ calls the function $approve(B, v)$, then the address $B$ can transfer at most $v$ tokens in total from the account of $A$ to other accounts. After this approval, account $B$ can transfer $v'$ tokens from the account of $A$ to the account of $C$ by calling the function \textit{transferFrom(A, C, v')}.

\subsection{AMM DEXs}

AMM DEXs are smart contracts on Ethereum. Users send messages to smart contract addresses to invoke functions for performing operations on the market. AMM DEXs support three kinds of operations regarding the exchange pair, i.e., creating the liquidity pool, adding/removing liquidity, and exchanging assets. We take Uniswap as an example to present these operations.

\subsubsection{Creating Liquidity Pools}

In AMM DEXs, exchanges between two tokens are conducted through a liquidity pool, i.e., a smart contract that keeps the pair of tokens. There are two participants involved in the market: the liquidity provider and the trader. Providers reserve their tokens in the liquidity pool, while traders exchange their capital with the other asset in the liquidity pool. Because providers contribute to the market liquidity, they benefit from the handling fees incurred with transactions in DEXs.

Assume we have two tokens $A$ and $B$ and we want to create a liquidity pool between $A$ and $B$ on Uniswap. We first send a message with the ERC20 smart contract address of $A$ and $B$ to the Uniswap smart contract to claim the creation of the liquidity pool $A\rightleftharpoons B$. The smart contract will then check whether the pool between $A$ and $B$ exists according to the addresses of the two tokens. If not, Uniswap smart contract will create a new liquidity pool $A\rightleftharpoons B$, i.e., a new smart contract for these two tokens, and record the information of these two tokens returned by the ERC20 functions, including name, symbol, and decimals.

\subsubsection{Adding/Removing Liquidity}

After creating the liquidity pool between $A$ and $B$, users can provide a pair of tokens to the liquidity pool for exchanges between two tokens. Users need to approve Uniswap address to transfer their $A$ token and $B$ token from the user's address to the liquidity pool address. When Uniswap contract receives a message of adding liquidity from the user, it will invoke functions in ERC20 contracts to transfer tokens from the user's address to the liquidity pool address.

In the first scenario, users can supply any amount of $A$ and $B$ to the liquidity pool and the pool will return $lp$ coins as certification of deposit. If the amounts of $A$ and $B$ provided by the user are $a$ and $b$, respectively, then the provider will get $a\times b$ lp tokens. Meanwhile, the total supply of lp token of $A\rightleftharpoons B$ pool is $l=a\times b$.

In the second scenario, a liquidity provider can reserve $\delta_a$ of its asset $A$ and $\delta_b$ of its asset $B$ in the liquidity pool simultaneously, where $\frac{\delta_a}{\delta_b}=\frac{a}{b}$. Then he will earn $\delta_{l} = l\cdot\frac{\delta_a}{a}$ lp tokens for the $A\rightleftharpoons B$ asset pair.

Liquidity providers can also remove their tokens from the liquidity pool. The amount of tokens users can redeem is related to the number of lp token they own. Assume an user has $\delta_p$ lp token and the liquidity of $A$ and $B$ are $a$ and $b$, respectively, then he can withdraw $\delta_a$ of $A$ and $\delta_b$ of $B$ from the $A\rightleftharpoons B$ pool, where $\frac{\delta_a}{a}=\frac{\delta_b}{b}\leq\frac{\delta_c}{c}$. The lp token he owns will also be destroyed in proportion to the money he redeems.

\subsubsection{Exchanging Assets}

In AMM DEXs, tokens are not exchanged between two traders but between the trader who initiates the transaction and liquidity pools. Therefore, the execution of exchanging assets is realized in two steps. First, the trader sends his tokens to the liquidity pool. Second, the liquidity pool computes the exchange rate and return the targeted token to the trader.

Assume a trader want to exchange $\delta_a$ of $A$ for $B$ token and the liquidity of $A$ and $B$ are $a$ and $b$. He first needs to let the Uniswap address to get the approval for transferring his $A$ token by invoking ERC20 contract functions. After receiving the exchange request message from the trader, Uniswap contract then transfers $\delta_a$ of $A$ to the liquidity pool address and returns $\delta_b$ of $B$ back to the trader.

The following equation always hold during the transaction: $a\cdot b = (a+\delta_a\cdot r_1)\cdot(b-\frac{\delta_b}{r_2})$, where $r_1$ and $r_2$ denote the transaction fee ratio in asset $A$ and $B$ respectively. In Uniswap, $r_1  = 0.997$ and $r_2=1$, which indicates that the transaction fee is equal to $3$\textperthousand$\cdot \delta_a$. The remaining liquidity in the pool equals to $(a+\delta_a, b-\frac{r_1\cdot r_2\cdot b\cdot\delta_a}{a+r_1\cdot\delta_a})$ and the amount of lp token does not change.

\subsection{Atomic Transactions}

An important issue of cyclic arbitrages is that traders can only get benefits if all the exchanges are executed successfully. Otherwise, if some external exchanges have not been executed, then traders may end up in a state of the deficit because the price of unsuccessful exchanges may change dramatically in the future.

In Etheurem, traders are allowed to issue atomic transactions. They can deploy smart contracts to executes several exchanges within one transaction. To avoid losses due to intermediate changes in exchange rates, arbitrageurs group cyclic transactions in a batch. Because Ethereum is a replicated state machine, the system state is changed only if the whole batch executes successfully. If the batch fails because a particular condition cannot be met (e.g., insufficient transaction fees, conflicting transactions, and prerequisites on the market state), the whole batch will not be executed.

An arbitrageur submits such a batch by deploying a proxy contract. A cyclic transaction is executed only if there is an income. While this seems risk-free for the cyclic arbitrageur, there are costs as well. In particular, the arbitrageur must pay a fee to the Uniswap pool liquidity providers of all the involved pools. On top of that, the Ethereum miners ask for a fee to execute the smart contract. Finally, there is a risk that the smart contract is not executed at all, in particular, if the cyclic trade was not profitable anymore at the time of execution (their smart contracts will check this). This may happen if the exchange rates changed, for instance, if another arbitrageur's (cyclic) trade was executed earlier. In this case, the miners will still ask for a fee.


\section{Data Description}

The main data for this project are trading data obtained from the largest CEXs (Binance) and DEXs (Uniswap V2).

Every successful trade in Uniswap is recorded on Ethereum blockchain. To collect trading data of Uniswap, we download all blocks of Ethereum and analyze from block 10000835, where Uniswap V2 has been deployed. We focus our analysis on the period after the appearance of these markets, i.e., from 20th May 2020 to xx .

Each trading pair in Uniswap is created by the UniswapV2Factory contact. We query this contract to get xxxx available trading pairs in Uniswap (until xx) and the contract address of these trading pairs.
For each successful exchange between two tokens, a \textbf{Swap} event will be generated by the trading pair contract and be included in the transaction receipt. The \textbf{Swap} event includes six parameters: \textbf{sender}, which is the initiator of the exchange; \textbf{to}, which is the receiver of the output tokens; \textbf{amount0In, amount1In, amount0Out, amount1Out}, which denote the amount of token0 spent by the initiator, the amount of token1 spent by the initiator, the amount of token0 received by the receiver, and the amount of token1 received by the receiver, respectively. 
If a trader exchanges $x$ amount of \textit{token0} for $y$ amount \textit{token1}, then $(amount0In, amount1In, amount0Out, amount1Out) =(x, 0, 0, y)$.
With the information contained in the \textbf{Swap} event, we can classify the direction and the amount of the exchange.

We write a script to collect all \textbf{Swap} events generated by the known xxxx pair contracts, which are included in transaction receipts on Ethereum. We obtain token exchanges happen in Uniswap between 04th May 2020 and xx. If several \textbf{Swap} events are involved in the same transaction receipt and the trading path of these exchanges can form a cycle, then we identify a successful cyclic transaction in Uniswap. 
To compute the successful rate of cyclic arbitrage, we also need the information of failed cyclic transactions. However, a \textbf{Swap} event is recorded in the transaction receipt only if the exchange has been executed successfully. Therefore, we statistic all failed transactions initiated by arbitrageurs who have performed cyclic transactions.
To perform a cyclic arbitrage, arbitrageurs will call smart contract functions with an encoded signature. These signatures always exist in transaction information on Ethereum, no matter the transaction executes successfully or not.
We collect signatures of all failed transactions in Ethereum and compare them with signatures of experienced arbitrageurs. If the signature of a failed transaction matches a successful one, we consider the failed transaction as a potential failed cyclic transaction.  

To better understand the relationship between prices in CEXs and DEXs, we obtain the trading data of CEXs by querying the Application Programming Interface (API) provided by Binance.
Binance provides tick-level data, including the timestamp of the transaction at the second and millisecond level, the price where the trade happened, the amount of the trade, and the trade direction (buy or sell initiated). We also collect minute-level Kline data, including open time, open price, close time, close price, high price, low price, volume, number of trades, and quote asset volume.
We restrict our attention to three cryptocurrency markets: bitcoin (BTC), ethereum (ETH), and uniswap (UNI). BTC and ETH are the most liquid and largest markets in CEXs, while the trading volume of them in CEXs is far more than those in DEXs. UNI is first issued in DEXs and the liquidity has gradually moved from DEXs to CEXs.

\section{Cyclic Arbitrages}

\subsection{Non-equilibrium of Exchange Rate}

\label{sec:non}

In Uniswap and many other AMM DEXs, users can create exchange markets for any pair of tokens, while the exchange rate between these two tokens only depends on the volume of tokens reserved in the smart contract. Assume we have three tokens $A, B, C$ and three liquidity pools between them. We want to exchange $A$ for $C$ in Uniswap markets. We can either trade in $A\rightleftharpoons C$ directly, or trade token $A$ for $B$ in $A\rightleftharpoons B$, then $B$ for $C$ in $B\rightleftharpoons C$ to complete the target transaction. The exchange rate between $A$ and $C$ through these two trading paths is not the same.

We denote $a_1$ and $b_1$ as amount of $A$ and $B$ in $A\rightleftharpoons B$, $b_2$ and $c_2$ as amount of $B$ and $C$ in $B\rightleftharpoons C$, and $c_3$ and $a_3$ as amount of $C$ and $A$ in $A\rightleftharpoons C$. We can directly exchange $\delta_a$ of token $A$ through the $A\rightleftharpoons C$ pool and earn $\delta_c$ of token $C$, where

\begin{equation}
    \begin{split}
    \delta_c = r_2\cdot(c_3-\frac{a_3\cdot c_3}{a_3+r_1\cdot\delta_a})= \frac{r_1\cdot r_2\cdot c_3\cdot\delta_a}{a_3+r_1\cdot\delta_a}
    \end{split}
    \label{equ:single}
\end{equation}

Or take token $B$ as an intermediate, where

\begin{equation}
\begin{split}
    \delta_c' = r_2\cdot(c_2-\frac{b_2\cdot c_2}{b_2+r_1\cdot \frac{r_1\cdot r_2\cdot b_1\cdot\delta_a}{a_1+r_1\cdot\delta_a}})
    = \frac{r_1\cdot r_2\cdot \frac{r_1\cdot r_2\cdot b_1 \cdot c_2}{b_2+r_1\cdot r_2\cdot b_1}\cdot\delta_a}{\frac{a_1 \cdot b_2}{b_2+r_1\cdot r_2\cdot b_1}+r_1\cdot\delta_a}
    \end{split}
    \label{equ:double}
\end{equation}

Compare Equation \ref{equ:single} and \ref{equ:double}, we can observe that the transaction through $A\rightleftharpoons B$ and $B\rightleftharpoons C$ is equivalent to an exchange of $\delta_a$ through liquidity pool $A'/C'$, where $a' = \frac{a_1 \cdot b_2}{b_2+r_1\cdot r_2\cdot b_1}$, and $c'=\frac{r_1\cdot r_2\cdot b_1 \cdot c_2}{b_2+r_1\cdot r_2\cdot b_1}$.

\begin{figure}[hpt]
\centering
\includegraphics[width=6cm]{ex1e}
\caption{Different exchange rates between Ethereum and Wrapped Bitcoin in block 11151407.}
\label{fig:exr}
\end{figure}

An example has been shown in Figure \ref{fig:exr}. We can trade 0.005 ETH for 0.0001466 WBTC through the $ETH\rightleftharpoons WBTC$ pool, or trade 0.005 ETH for 0.1694 LINK in the $ETH\rightleftharpoons LINK$ pool first and then obtain 0.0001496 WBTC through the $LINK\rightleftharpoons WBTC$ pool. The direct exchange rate between ETH and WBTC is 34.1:1, while if we use LINK as an intermediate, the exchange rate is 33.4:1.

Todo: arbitrage index across different markets.

\subsection{Cyclic Arbitrage Transactions}

The unbalanced exchange rates in the market enable arbitrageurs to engage in creation-redemption to benefit themselves. In other words, cyclic transactions exploit divergent exchange rates between markets. Arbitrageurs can submit a series of transactions that start and end with the same currency, i.e., $A\rightarrow B\rightarrow C\rightarrow D \ldots \rightarrow A$.

\begin{figure}[hpt]
\centering
\includegraphics[width=6cm]{ex2e}
\caption{An example cyclic transaction in Uniswap V2, executed on October 30th, 2020.}
    \label{fig:ring}
\end{figure}

Figure \ref{fig:ring} shows an example of a cyclic arbitrage executed on October 30th, 2020. The arbitrageur traded 285.71 USDC in Uniswap V2 through four different liquidity pools across USD Coin, Tether USD, Seal Finance, Keep3rV1, and finally received 303.68 USDC. The arbitrageur's income was 17.97 USDC.

Whether a cyclic transaction is profitable depends on the exchange rates between tokens, which are predefined by the market mechanism. 
Assume an arbitrageur trades $\delta_a$ of token $A$ across the market of three tokens $A$, $B$, and $C$. 
He has two possible trading strategies, namely exchanging $\delta_a$ through $A\rightarrow B\rightarrow C\rightarrow A$ path or $A\rightarrow C\rightarrow B\rightarrow A$ path. We denote $U_{ABCA}$ and $U_{ACBA}$ as the utility of these two strategies, respectively, where,

\begin{equation}
    \begin{split}
    U_{ABCA} = \delta_a' - \delta_a=(\frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot b_1\cdot c_2\cdot a_3}{b_2\cdot c_3+r_1\cdot r_2\cdot b_1\cdot c_3+r_1^2\cdot r_2^2\cdot b_1\cdot c_2}}{\frac{a_1\cdot b_2\cdot c_3}{b_2\cdot c_3+r_1\cdot r_2\cdot b_1\cdot c_3+r_1^2\cdot r_2^2\cdot b_1\cdot c_2}+r_1\cdot\delta_a}-1)\cdot \delta_a
    \end{split}
    \label{equ:31}
\end{equation}

\begin{equation}
    \begin{split}
    U_{ACBA} = \delta_a' - \delta_a=(\frac{r_1\cdot r_2\cdot \frac{r_1^2\cdot r_2^2 \cdot c_3\cdot b_2\cdot a_1}{c_2\cdot b_1+r_1\cdot r_2\cdot c_3\cdot b_1+r_1^2\cdot r_2^2\cdot c_3\cdot b_2}}{\frac{a_3\cdot c_2\cdot b_1}{c_2\cdot b_1+r_1\cdot r_2\cdot c_3\cdot b_1+r_1^2\cdot r_2^2\cdot c_3\cdot b_2}+r_1\cdot\delta_a}-1)\cdot \delta_a
    \end{split}
    \label{equ:32}
\end{equation}

The arbitrageur can benefit from the cyclic transaction if either $U_{ABCA}>0$ or $U_{ACBA}>0$, which only depends on the amount of tokens stored in the liquidity pools and the amount of tokens that traders would like to exchange. 
When an Ethereum block is published, the information of liquidity pools' balance is also available to all traders. 
Therefore, traders can quickly determine whether there is an opportunity for profitable cyclic transactions in the market by monitoring public information.

\begin{figure}[hpt]
\begin{minipage}[t]{0.49\linewidth}
\centering
\includegraphics[width=6cm]{start_token}
\caption{Tokens for exchange in cyclic transactions.}
\label{fig:starttoken}
\end{minipage}
\begin{minipage}[t]{0.49\linewidth}
\centering
    \input{daily_revenue}
    \caption{Revenue of cyclic transactions in Uniswap V2 (ETH). The black line shows a 7-day moving average of market size. The dotted orange line shows the cumulative market size. The scatter plot coloring indicates the number of daily cyclic arbitrage transactions.}
    \label{fig:revenue}
\end{minipage}
\end{figure}

Until xx, we find xxx arbitrageurs performing xxx cyclic transactions in Uniswap, generating xxx ETH (xxx USD) revenue.
%We found 199 arbitrage contracts, 136569 successfully executed arbitrage transactions generated 23092.46 ETH revenue, which is about 12720000 US Dollars at the time of writing, 5202.30 ETH cost as gas fee to execute these transactions, and 68868 failed transactions cost 2554.53 ETH in gas.
More than 98\% of cyclic transactions start with ETH (Figure \ref{fig:starttoken}), which is the naive cryptocurrency of Ethereum, while other starting tokens are mainly stable coins (the value of a stable token is pegged to USD) or tokens with a high price.

The market price of tokens in DEXs is always unbalanced, and arbitrageurs do not need any additional information other than Ethereum blocks to find profitable opportunities. 
Therefore, the market size of cyclic arbitrages has been gradually increasing since 04th May, when Uniswap V2 first deployed on block 10000835. Figure \ref{fig:revenue} shows the cyclic arbitrage market size, denominated in ETH.

Arbitrageurs started to perform cyclic arbitrage from 20th May, two weeks after the start of Uniswap V2.
From 20th May to 1st August, the market has been growing in daily revenue, reaching 100 ETH. The daily number of cyclic transactions climbs to 500 during the two months period.
At this stage, arbitrageurs in the market performed 124 cyclic transactions for a profit of 0.12 ETH (170 USD) per transaction on average, summing up to 14.39 ETH revenue in total daily in the market.

Todo:average revenue of cyclic transactions each day

Later the market has grown into a more mature stage, while more arbitrageurs joined the market and more revenue has been gained by arbitrageurs. The daily number of cyclic transactions reaches 2500 and the daily revenue reaches 1000 ETH.
However, the average revenue of cyclic transaction does not vary too far, keeping 0.17 ETH (250 USD).
%Arbitrageurs earn 149.79 ETH on average per day.  870 transactions

\begin{figure*}
    \centering
    \input{top_bots}
    \caption{Top bots profit}
    \label{fig:topbots}
\end{figure*}

%Figure \ref{fig:topbots} shows the daily arbitrage profit of the top 10 bots we observed with highest total profit. The addresses showed are arbitrage contract addresses, not external owned accounts(EOA), because an arbitrageur may use multiple EOAs to initiate arbitrage transactions so that they can capture as many arbitrage opportunities as they can. Here the profit equals revenue subtract gas cost, so there may be negative profit arbitrage transactions, as we can see in the graph, from 06-09 to 06-19, the black line(market total profit) is below the blue dotted line, means there are bots making negative profit arbitrage transactions during this period. We can see that the 0x860bd2... bot(blue dotted line) dominates the market at most of the time.

\subsection{Existence of Arbitrage Opportunities}

There are around 2000 trading pairs in Uniswap V2, and the trading cycle can be arbitrary long. With Equation \ref{equ:31} and \ref{equ:32}, arbitrageurs can only know whether a cyclic transaction is profitable. However, it is not clear whether there are arbitrage opportunities within the million of trading cycles. We find that based on the market state published on Ethereum blocks, traders can easily determine whether a profitable cyclic transaction exists.

\begin{lemma}
For a given cycle $A\rightarrow B^1\rightarrow \ldots \rightarrow B^n\rightarrow A$ with $n+1$ tokens, there exists arbitrage opportunity for the cyclic transaction if $\frac{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}<r_1^{n+1}\cdot r_2^{n+1}$. Meanwhile, the arbitrage cannot benefit from the reversed direction $A\rightarrow B^n\rightarrow \ldots \rightarrow B^1\rightarrow A$ for cyclic transactions.
\label{lemma:th}
\end{lemma}

We first give a general expression of cyclic transactions with more than three tokens.

\begin{lemma}
For a cyclic transaction through a path with $n+1$ edges $A\rightarrow B^1\rightarrow B^2\rightarrow \ldots \rightarrow B^n\rightarrow A$, the first deviation of the utility function at $\delta_a=0$ is $\frac{\partial U}{\partial \delta_a}\bigg|_{\delta_a = 0}=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1$.
\label{lemma:2}
\end{lemma}

\begin{proof}
We prove this lemma by induction. We first show it is correct when $n=2$.

We take the utility function of a cyclic transaction of three tokens as shown in Equation \ref{equ:31} and compute the first deviation of the function,

\begin{equation}
    \frac{\partial U_{AB^1B^2A}}{\partial \delta_a}\bigg|_{\delta_a = 0}=\frac{r_{1}^3\cdot r_{2}^3\cdot a_{3}\cdot b^1_{1}\cdot b^2_{2}}{a_{1}\cdot b^1_{2}\cdot b^2_{3}} -1
\end{equation}

For $n>2$, the inductive hypothesis is that the equation is true for $n$: 

$\frac{\partial U}{\partial \delta_a}\bigg|_{\delta_a = 0}=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1$.

The inductive step is to prove the equation for $n+1$:

If we exchange $\delta_a$ through $A/B^1$ pool to get $\delta_b^1$, and obtain $\delta_b^2$ from $B^1/B^2$ by trading $\delta_b^1$ right after, these two atomic transactions can is equivalent to a single transaction with $\delta_x$ in a virtual pool $A_v/B_v$, where $a_v = \frac{a_1 \cdot b^1_2}{b^1_2+r_1\cdot r_2\cdot b^1_1}$, and $b_v=\frac{r_1\cdot r_2\cdot b^1_1 \cdot b^2_2}{b^1_2+r_1\cdot r_2\cdot b^1_1}$.

We assume that the statement is correct for any $n$-path cyclic transaction. Consider a cyclic transaction through a $n+1$-path $A\rightarrow B^1\rightarrow B^2\rightarrow \ldots \rightarrow B^n\rightarrow A$, which is equivalent to a $n$-path cyclic transaction through $A_v\rightarrow B_v\rightarrow \ldots \rightarrow B^n\rightarrow X$, where the first deviation of the utility function at $\delta_a=0$ is,

\begin{equation}
    \begin{split}
        \frac{\partial U}{\partial \delta_a}\bigg|_{\delta_a = 0}&=\frac{r_1^{n}\cdot r_2^{n}\cdot a_{n+1}\cdot b_v\cdot \ldots\cdot b^n_n}{a_v\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1\\
        &=\frac{r_1^{n}\cdot r_2^{n}\cdot a_{n+1}\cdot \frac{r_1\cdot r_2\cdot b^1_1 \cdot b^2_2}{b^1_2+r_1\cdot r_2\cdot b^1_1}\cdot \ldots\cdot b^n_n}{\frac{a_1 \cdot b^1_2}{b^1_2+r_1\cdot r_2\cdot b^1_1}\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1\\
        &=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1
    \end{split}
\end{equation}

By the principle of mathematical induction: the first deviation of the utility function at $\delta_a=0$ is $\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1$, for any $n\geq 2$.

\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:th}]

Assume that we would like to exchange $\delta_a$ of token $A$ through the cycle. When $\delta_a = 0$, both the value of $U_{AB^1B^nA}$ and the value of $U_{AB^nB^1A}$ are 0.

Then we consider the first and the second derivative of the utility function at $\delta_a = 0$.

\begin{equation}
    \frac{\partial U_{AB^1B^nA}}{\partial \delta_a}\bigg|_{\delta_a = 0}=\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}-1
\end{equation}

If arbitrageurs can make profit in this trading direction, then, 

\begin{equation}
    \begin{split}
        0&<\frac{\partial U_{AB^1B^nA}}{\partial \delta_a}\bigg|_{\delta_a = 0}\\
        \frac{1}{r_1^{n+1}\cdot r_2^{n+1}}&<\frac{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}\\
        \frac{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}&<r_1^{n+1}\cdot r_2^{n+1}
    \end{split}
\end{equation},

which implies that $\frac{r_1^{n+1}\cdot r_2^{n+1}\cdot a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}<1$, then $\frac{\partial U_{AB^nB^1A}}{\partial \delta_a}\bigg|_{\delta_a = 0}<0$.

By computing the second derivative of $U_{AB^nB^1A}$, we know that $\frac{\partial^2 }{\partial \delta_a^2}U_{AB^nB^1A}$ is negative for all $\delta_a\in R^+$. $U_{AB^nB^1A}$ is a monotone decreasing function in its domain, and the maximum value of $U_{AB^nB^1A}$ is 0 at $\delta_a=0$. Therefore, there is no opportunity for arbitrage through the reversed direction $A\rightarrow B^n\rightarrow \ldots \rightarrow B^1\rightarrow A$ for cyclic transactions.

Arbitrageurs cannot benefit from trading $\delta_a$ through $A\rightarrow B^n\rightarrow \ldots \rightarrow B^1\rightarrow A$, sequentially. Therefore, arbitrageurs have at most one direction to benefit themselves with cyclic transactions.

\end{proof}

Lemma \ref{lemma:th} suggests that the longer the cycle, the more restricted requirement is imposed on the exchange rate ratio across markets for profitable cyclic transactions.
Figure \ref{fig:len} shows the statistics of length of cyclic transactions in Uniswap V2. Three is the minimum length of a cyclic transactions. Therefore, the majority (more than 90\%) of cyclic transactions is applied with markets of three tokens. 

\begin{figure}
    \centering
    \includegraphics[width=8cm]{ring_length}
    \caption{Length of cyclic transactions.}
    \label{fig:len}
\end{figure}

We can observe that the number of cyclic transactions decreases as the cycle length increases.
Why arbitrageurs prefer cycles with short length? There are three main reasons.

First, as we showed in Lemma \ref{lemma:th}, the required product of exchange rate decreases exponentially with the length of cycles. For example, in Uniswap V2, if we exchange token $A$ through a 3-path cycle, then the product of three exchange rates should be less than 0.991 for a profitable cyclic transaction. However, if the length of the cycle is 6, then the product of six exchange rates should be less than 0.982, which is much harder than finding arbitrage opportunities in markets with fewer tokens.

Second, arbitrageurs can easily benefit from trading in markets with three tokens. 
No matter how many cyclic transactions appear on markets, the average revenue of each cyclic transaction keeps around 0.15 ETH. Arbitrageurs do not aim to find the maximal arbitrage opportunity in the market, while more than xx\% of cyclic transactions aim to achieve revenue less than 0.2 ETH.
As shown in Figure xx, there are already many arbitrage opportunities in markets with three tokens.
Therefore, arbitrageurs are more likely to search for arbitrage opportunities in the market with fewer tokens first, which can already satisfy their trading demand.

Third, long cyclic transactions are more susceptible to market changes. 
There is a latency between arbitrageurs submitting transactions and the execution of the transactions.
During this period, other market trade changes the exchange rate between tokens. 
Because long cyclic transactions are involved with more tokens and more trading markets, the exchange rate is more likely to deviate from the expected rate because of the influence of other trade. 
Therefore, to reduce this risk, arbitrageurs prefer trading through shorter cycles.

\section{Cost of Cyclic Arbitrages}

Although arbitrageurs submit their transaction requests as soon as they observe an opportunity for cyclic arbitrages, there is still a risk that the arbitrageurs will not benefit from the transactions. 
Miners will collect transactions that have not been executed from the Ethereum network and order them in the newly generated block according to their own wishes (normally according to the gas price). Some transactions may be executed prior to the cyclic transactions. 
Therefore, when the cyclic transaction executes, the exchange rate might deviate far away from when the trader creates the transaction.

Ehtereum allows arbitrageurs to hedge such risks by deploying proxy contracts. Arbitrageurs can group the cyclic transactions in a batch. Because Ethereum is a replicated state machine, the system state is changed if the whole batch executes successfully. If the batch fails because a particular condition cannot be met (e.g., insufficient transaction fees, conflicting transactions, and prerequisites on the market state), the whole batch will not be executed. The system state will be backdated to the state when the batch has not been started. Therefore, the cyclic transaction is valid only if there is an income of the transaction.

While this seems risk-free for the cyclic arbitrageur, there are costs as well. In particular, the arbitrageur must pay a fee to the Uniswap pool liquidity providers of all the involved pools. On top of that, the Ethereum miners ask for a fee to execute the smart contract. Finally, there is a risk that the smart contract is not executed at all, in particular, if the cyclic trade was not profitable anymore at the time of execution (their smart contracts will check this). This may happen if the exchange rates changed, for instance, if another arbitrageur's (cyclic) trade was executed earlier. In this case, the miners will still ask for a fee.

Todo: cost distribution for successful transactions, cost distribution for failed transactions, profit distributions

What are the costs of the arbitrageurs? We count the success rate for those arbitrageurs who have performed more than 100 cyclic transactions. With the public Ethereum information, we cannot distinguish whether a failed arbitrageur transaction was indeed a failed cyclic batch. With this conservative assumption, the success rate of arbitrageurs is still high, i.e., $\frac{130490}{163962}=79.59\%$. Figure \ref{fig:revenue} shows the profitability of the successfully executed arbitrage transactions. Only 6816 out of 134962 transactions had a negative profit because their trading revenue did cover the mining cost. The entire revenue of cyclic arbitrageurs was  17,632.57 ETH.


\begin{figure}
    \centering
    \includegraphics[width=8cm]{profitability}
    \caption{Profit/Revenue distribution}
    \label{fig:hist}
\end{figure}

Figure \ref{fig:hist} shows the profitability of the successfully executed arbitrage transactions. 131358 transactions generate a profit in the range of -0.1 ETH to 0.7 ETH, which is more than 96\% of the total number of successfully executed arbitrages. Most of the transactions generate less than 0.1 ETH profit, and some even have negative profit because their revenue cannot cover the gas cost.
 
\begin{figure*}
    \centering
    \input{top10_paths}
    \caption{Top paths}
    \label{fig:toppaths}
\end{figure*}

\iffalse
\begin{figure*}
    \centering
    \input{toppath_pairs}
    \caption{Top path pairs}
    \label{fig:toppath_pairs}
\end{figure*}
\fi


Figure \ref{fig:toppaths} shows the top 10 rings the arbitrageurs execute their arbitrage transactions. Everyone can issue a token on Ethereum and add a trading pair on Uniswap for the token, some tokens are more active than others during a certain period of time, resulting in more arbitrage opportunities, after that, the price becomes more stable and the market is less active, thus less arbitrage opportunities. Most of the rings showed in this figure follow this pattern, token listed, market is active and price is fluctuating heavily, drawing more arbitrageurs, then gradually stabilize, then new tokens listed, repeat this process over and over again.

\begin{figure*}
    \centering
    \input{gas_trend}
    \caption{Gas Trend}
    \label{fig:gastrend}
\end{figure*}

%Figure \ref{fig:gastrend} shows the gas trend of ring arbitrage transactions, the y axis is the mean gas used per arbitrage transactions, and the coloring indicates the mean gas price, we can see a slightly down trend in the figure, and the mean gas used is gathering over time, which means the arbitrageurs are optimizing their gas cost. The gas price was very high in August and September, we can see there are two sharp down trends around the highest gas price days, because gas price affects the profitability of the arbitrage, arbitrage transactions cost more fees (gas * gas price) when gas price is high, the arbitrageurs have to optimize their gas used per transaction in order to make a profit, and those who failed to optimize the gas cost have to stop the arbitrage, leaving only the optimized ones in the market, so we can see the sharp down trend in mean gas used per arbitrage.


\section{Interactions with Other Participants}

To better understand how cyclic arbitrages influence the market, we consider the market behavior and profits of other participants (normal traders and liquidity providers). 
We study a theoretical model of cyclic arbitrage and find that cyclic arbitrage balances the exchange rates across different pools. This is good for traders (who trade in a fair market), and as a consequence, also for the liquidity pool providers (since the increased trust in the system will also increase the number of trades, and as such, their income from fees).
Then we analyze the behavior of normal traders and liquidity providers when cyclic arbitrages occur with varying frequency.

\subsection{Market Price Balance and Normal Trades}

First, we consider how cyclic transactions influence the market price of tokens, which is important for normal traders who use DEXs to exchange assets. Arbitrageurs aim to eliminate the price differences on markets and benefit themselves from trading across markets. Cyclic transactions can effectively balance the price between tokens through different trading paths and provide fair markets for normal traders.

\begin{lemma}
The market price after cyclic transactions is more balanced than the price before the cyclic transactions. In other words, there are fewer arbitrage opportunities after the cyclic transactions.
\end{lemma}

\begin{proof}
Consider a cyclic transaction through trading path $\delta_a$ through $A\rightarrow B^n\rightarrow \ldots \rightarrow B^1\rightarrow A$.

A cyclic transaction is profitable through the path if the product of exchange rates before the transaction satisfies $\frac{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}<r_1^{n+1}\cdot r_2^{n+1}$.

After the transaction, the product have to satisfy $\frac{(a_1+\delta_a)\cdot (b^1_2+\delta_{b^1})\cdot (b^2_3+\delta_{b^2})\cdot\ldots\cdot (b^n_{n+1}+\delta_{b^n}}{(a_{n+1}-\delta_a')\cdot (b^1_1-\delta{b^1})\cdot (b^2_2-\delta_{b^2})\cdot \ldots\cdot b^n_n}<r_1^{n+1}\cdot r_2^{n+1}$. Otherwise, there is no income for arbitrageurs from this transaction. Thus, this cyclic transaction will not be executed.

Before the cyclic transaction, for two tokens in the market, such as $A$ and $B_i$, there are two market exchange rates between them, namely $\frac{a_1}{b^1_1}\cdot \frac{b^1_2}{b^2_2}\cdot\ldots\cdot\frac{b^{i-1}_i}{b^i_i}$ and $\frac{a_{n+1}}{b^n_{n+1}}\cdot \frac{b^n_n}{b^{n-1}_n}\cdot\ldots\cdot\frac{b^{i+1}_{i+1}}{b^i_{i+1}}$. The arbitrage index of these two prices is exactly $\frac{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}$, which is larger than $\frac{1}{r_1^{n+1}\cdot r_2^{n+1}}$.

Similarly, after the cyclic transaction, the arbitrage index of two market exchange prices between $A$ and $B_i$ moves to the product of the exchange rates among market, which is less than $\frac{1}{r_1^{n+1}\cdot r_2^{n+1}}$.

Therefore, the market price is more balanced after cyclic transactions.

\end{proof}

Todo: normal trades vs cyclic transactions

\subsection{Profit for Liquidity Providers}

Other than traders, liquidity providers also perform an important role in DEXs. Liquidity providers reserve their tokens in the smart contracts (liquidity pools) of DEXs, which enables traders to exchange their assets with the markets. There is no need for a third-party to managing transactions on DEXs because all exchanges can be executed following the predefined mechanism.

Liquidity providers contribute to the one-sided trading in DEXs. Exchanges will be executed instantly once been recorded in the blocks of Ethereum. Traders are trading with the liquidity pools without the participation of another trader who wants an exchange of the reversed direction. 

Moreover, the contributions of liquidity providers also influence price stability. Assume there are two markets between $A$ and $B$. In the first market, the liquidity pool reserves $a=10000$ and $b=1000$, while in the second market, the liquidity pool reserves $a'=100$ and $b'=10$. The exchange rates between $A$ and $B$ are $10:1$ in both markets. However, after an exchange of 10 $A$ with $B$, the exchange rate in the first market moves to $\frac{10010}{999}=10.02$, while the exchange rate in the second market moves to $\frac{110}{9.1}=12.1$. Therefore, the exchange rate in the first market is more stable because of the contributions of liquidity providers.

To reward liquidity providers and attract more liquidity providers to reserve their money in liquidity pools, DEXs pay a transaction fee to liquidity providers for each transaction. In Uniswap V2, 0.3\% of trading tokens will remain in the liquidity pool, which can be withdrawn by liquidity providers.

However, other than normal traders, cyclic arbitrageurs do not care about the exchange rate between two tokens in a certain market. They perform cyclic transactions if the market price is not balanced across different markets. Therefore, it is possible that cyclic arbitrageurs move the exchange rate between tokens far away from what other traders expect. We find that cyclic transactions can increase the number of trading in DEXs, resulting in more transaction fees to liquidity providers.

\begin{lemma}
    If the market is efficient, liquidity providers gain more transaction fees if cyclic transactions appear during the convergence of the market prices.
\end{lemma}


\begin{proof}

Consider the exchange rate between tokens $A$ and $B$ is $\frac{a}{b} = r$ at time point $t$, and rational traders would like to move this rate to $r'$ by a transaction $T$.

Assume there is cyclic transaction $T^c$ happens at $t$ and moves the exchange rate to $r_c$. We analyze how this cyclic transaction changes the profit of liquidity providers.

If $r_c=r'$, which means that $T^c$ already moves the market price as other traders want. There is no need for an additional transaction $T$. Cyclic transaction $T^c$ does not change the profit of liquidity providers while it just substitutes of the original trade $T$.

Otherwise, $r_c\neq r'$, which means there will be another transaction $T'$ to move the market price to $r'$. Then we compare the profit of liquidity providers with $T$, and with the combination of $T^c$ and $T'$.

We assume that $T=(+\delta_{a}, -\delta_b)$, where traders would like to exchange $\delta_{a}$ of $A$ with $\delta_{b}$ of $B$ from the market. There are three scenarios according to the cyclic transaction $T^c$ and $T'$.

\begin{itemize}
    \item $T^c=(+\delta_{a}^{c}, -\delta_b^{c})$ and $T'=(-\delta_a', +\delta_b')$: 
    We can deduct that $\delta_{a}^{c}>\delta_{a}$. It turns out that $T^c$ leaves $\delta_{a}^{c}\cdot(1-r_1)$ of token $A$ as the transaction fee in the liquidity pool, which is more than what $T$ can contribute to the liquidity pool. Therefore, liquidity providers earn more transaction fees because of the cyclic transaction.
    
    \item $T^c=(-\delta_{a}^{c}, +\delta_b^{c})$ and $T'=(+\delta_a', -\delta_b')$: 
    We can deduct that $\delta_a'>\delta_a$. It turns out that $T'$ leaves $\delta_a'\cdot(1-r_1)$ of token $A$ as the transaction fee in the liquidity pool, which is more than what $T$ can contribute to the liquidity pool. Therefore, liquidity providers earn more transaction fees because of the cyclic transaction.
    
    \item $T^c=(+\delta_{a}^{c}, -\delta_b^{c})$ and $T'=(+\delta_a', -\delta_b')$: 
    The cyclic transaction  $T^c$ leaves $\delta_{a}^{c}\cdot(1-r_1)$ of token $A$ as transaction fee in the liquidity pool. Because the product of tokens' volume is a constant in Uniswap, after the cyclic transaction $T^c$, the product of tokens' volume is increased by $\delta_{a}^c\cdot(1-r_1)\cdot(b-\delta_b^c)$. Meanwhile, the exchange rates between $A$ and $B$ after $T$ and $T'$ are the same. Therefore, $T^c$ and $T'$ leave more transaction fees in the liquidity pool then $T$.
\end{itemize}
\end{proof}

Todo: size of liquidity pool/revenue of liquidity providers vs cyclic transactions.

\section{Arbitrage Across Different DEXs}
Todo: arbitrage index between Uni/Sushi/Curve

\section{Price Movement From CEXs to DEXs}
Todo: market size comparison between CEXs and DEXs




\subsection{Successful Transactions}


\autoref{fig:cos} shows the distribution of the gas fee of successful cyclic transactions.
Notice that a cyclic transaction might involve several cycles. However, it is impossible to distinguish the gas fee for each cycle separately. Therefore, we only consider the net profit of the entire transaction. More than half of transactions spend less than 0.02 ETH as the gas fee to miners, and only 11.8\% of transactions spend more than 0.05 ETH to execute the transaction. The gas fee (7,869.14 ETH) only accounts for 24.9\% of the total revenue (31,727.11 ETH) of cyclic transactions. \autoref{fig:hist} compares arbitrage income and net profit for cyclic arbitrages. Only 6.7\% of cyclic arbitrages result in negative profits. Gas fees drive revenue per cyclic arbitrage from 0.1-0.3 ETH gross revenue to 0-0.1 ETH net profit, where the majority of cyclic arbitrages (68.2\%) falling in this range.
\iffalse
\begin{figure}
    \centering
    \input{gas_trend}
    \setcaptionwidth{0.9\linewidth}
    \caption{Trends in quantity of gas consumption per cyclic transaction over time.}
    \label{fig:gastrend}
\end{figure}

\begin{figure}
    \centering
    \input{gas_price}
    \setcaptionwidth{0.9\linewidth}
    \caption{Trends in gas price of cyclic transaction over time.}
    \label{fig:gasprice}
\end{figure}

The cost of a successful cyclic transaction (gas fee) is determined by the gas price and the amount of gas used by miners to run the contract (gas fee = gas price $\times$ gas consumption).
To minimize the gas fee, arbitrageurs can either decrease the gas price (may result in lower priority of their transactions and longer waiting time for miners to execute), or optimize the executing efficiency of their transaction.
\autoref{fig:gastrend} shows the optimization of transaction execution over time.
The average gas consumption per transaction has been decreasing from 400,000 to 250,000 between May and January. Meanwhile, the gas price is extremely high in August and September (\autoref{fig:gastrend}), resulting in a sharp downtrend of the mean gas used (yellow and red plots are lower than blue plots at similar time points). Because if arbitrageurs want a positive profit when the gas price is very high, they have to optimize their gas used per transaction during the period.
\fi
%Figure \autoref{fig:gastrend} shows the gas trend of ring arbitrage transactions, the y axis is the mean gas used per arbitrage transactions, and the coloring indicates the mean gas price, we can see a slightly down trend in the figure, and the mean gas used is gathering over time, which means the arbitrageurs are optimizing their gas cost. The gas price was very high in August and September, we can see there are two sharp down trends around the highest gas price days, because gas price affects the profitability of the arbitrage, arbitrage transactions cost more fees (gas * gas price) when gas price is high, the arbitrageurs have to optimize their gas used per transaction in order to make a profit, and those who failed to optimize the gas cost have to stop the arbitrage, leaving only the optimized ones in the market, so we can see the sharp down trend in mean gas used per arbitrage.


\section{Impact on Market Prices and Participants}

In this section, we consider how cyclic arbitrages change the market and influence on other market participants (normal traders and liquidity providers). 
Cyclic arbitrages balance the exchange rates across different pools. This is good for traders (who trade in a fair market), and as a consequence, also for the liquidity pool providers (since the increased trust in the system will also increase the number of trades, and as such, their income from transaction fees).

\subsection{Market Price Balance}

First, we consider how cyclic arbitrages change the market price of tokens. Cyclic arbitrages can effectively balance the price between tokens through different trading paths and provide fair markets for normal traders. We find that a cyclic arbitrage with positive utility can always balance the market price (\autoref{sec:lp}). In other words, the market price after cyclic transactions is more balanced than the price before the cyclic transactions.

\autoref{fig:rate} shows the change of the arbitrage index within the cycles before and after the transaction. Apart from what we have shown in the figure, more than one-third of cyclic transactions happen when the arbitrage index is larger than 1.1 (119,621 out of 285,217). Our result shows that the market price is always balanced after cyclic transactions, where the arbitrage index of these cycles always becomes smaller than the previous index. Normal traders can exchange their assets in a more fair market. Moreover, the closer the trading volume is to the optimal input volume, the more balanced the exchange rates are. Therefore, our results indicate the high efficiency of cyclic arbitrages in Uniswap.

Even though arbitrageurs may not balance the market prices perfectly and remain price deviations in the market, most of them (147,011 out of 285,217) do not leave any cyclic arbitrage opportunity. The arbitrage index is smaller than $1.003^3$ after these cyclic arbitrages, which is the minimum requirement on the arbitrage index for a positive revenue of cyclic transactions of length 3. 

\subsection{Influence on Liquidity Providers}

Other than traders, liquidity providers also perform an important role in DEXes. Liquidity providers reserve their tokens in liquidity pools, enabling traders to exchange their assets with the pools. Liquidity providers contribute to the one-sided trading mechanism of DEXes. Traders are trading with the liquidity pools without the participation of another trader. 

Moreover, the contributions of liquidity providers also influence price stability. Assume there are two markets between $A$ and $B$. In the first market, the liquidity pool reserves $a=10000$ and $b=1000$, while in the second market, the liquidity pool reserves $a'=100$ and $b'=10$. The exchange rates between $A$ and $B$ are $10:1$ in both markets. After an exchange of 10 $A$ with $B$, the exchange rate in the first market moves to $\frac{10010}{999}=10.02$, while the exchange rate in the second market moves to $\frac{110}{9.1}=12.1$. The exchange rate in the first market is more stable than the second because of the contributions of liquidity providers.

To reward liquidity providers and attract more liquidity providers to reserve their money in liquidity pools, traders pay a transaction fee to liquidity providers for each transaction. In Uniswap, 0.3\% of trading volume will remain in the liquidity pool as the transaction fee.

When playing the arbitrage strategy, cyclic arbitrageurs do not care about the exact exchange rate between two tokens in a liquidity pool but whether the market price is balanced across different pools. Cyclic arbitrageurs may move the exchange rate between tokens away from what other traders expect. Other traders have to perform more trades in the market to drive the exchange rate between tokens to the price they have in mind (\autoref{sec:lp}). Thus, cyclic transactions can increase the number of trading in DEXes, resulting in more transaction fees to liquidity providers.

We analyze the relationship between the daily change of \textit{lp} tokens (represents the total contribution of liquidity providers) and the daily number of cyclic transactions in six liquidity pools where cyclic arbitrages always happen (\autoref{sec:popular}), i.e. $ETH\rightleftharpoons YAM$, $ETH\rightleftharpoons BADGER$, $ETH\rightleftharpoons REVV$, $ETH\rightleftharpoons RWS$, $ETH\rightleftharpoons HEGIC$, $ETH\rightleftharpoons XFI$. We find that the correlation coefficients are almost zero for the first four pools and are around 0.3 for the last two pools.

In real markets, the behavior of liquidity providers is influenced by many other factors, such as the price of tokens in other exchanges, the trading volume through the liquidity pool, and other liquidity providers' market performance. Moreover, the majority of liquidity providers lack information about cyclic transactions and how these transactions benefit themselves. Even though liquidity providers' behaviors seem highly likely irrelevant to the involvement of cyclic arbitrageurs, we find that cyclic arbitrages do not hurt liquidity providers' benefits (\autoref{sec:lp}). The participant of cyclic arbitrageurs does not influence liquidity providers' engagement in DEXes.
\iffalse
\section{Arbitrage Across Different DEXes}

Price deviations not only appear within the same DEX, but also spread across different DEXs. Even for the same trading pair of tokens, exchange rates in different DEXes are also not the same, enabling traders to perform more cyclic arbitrages across liquidity pools of multiple DEXes, even arbitrages with cycles of length 2.

We collect the block-wise exchange rate (the ratio of token volume reserved in the liquidity pool) of fifteen popular trading pairs in both Uniswap and Sushiswap and compute the block-wise arbitrage index between two exchanges. The arbitrage index of a trading pair is calculated by dividing the high exchange rate between the two markets by the low exchange rate.

\begin{figure}
    \centering
    \includegraphics[width = 1\textwidth]{sushi.png}
    \caption{Arbitrage index of Uniswap/Sushiswap pairs}
    \label{fig:sushi}
\end{figure}

\autoref{fig:sushi} shows the arbitrage index of these 15 token pairs between the trading pool in Uniswap and Sushiswap over time. From Lemma \ref{lemma:th}, we know that cyclic arbitrages of length 2 are profitable if the arbitrage index is larger than 1.006. One-third of these 15 token pairs yield an average arbitrage index larger than the threshold, and 12\% of block-wise arbitrage index among all these token pairs is larger than the arbitrage threshold, indicating great opportunities for cyclic arbitrages across different DEXes. Here we only collect the 15 largest liquidity pools in Uniswap and Sushiswap, where the trades frequently happen across two DEXes. The market price is expected to be balanced in these pools. We can infer that for other pools with less liquidity, where not many trades perform across different DEXes, the arbitrage index may be higher than what we show here.
\fi
\section{Discussion}

\subsection{Arbitrage in DEXes and CEXes}

Cyclic arbitrage opportunities appear in CEXes of cryptocurrencies when there are price deviations across different markets. For example, when the price of bitcoin in a US market (such as Coinbase) is above the price in a Japanese market (such as bitFlyer), an arbitrageur can buy bitcoins in Japan, sell them in the US, and then exchange US dollars for Japanese YEN~\cite{makarov2020trading} (trading through a cycle of Japanese YEN, bitcoin, and US dollars). However, there are many constraints to arbitrage in CEXes, such as transaction costs between different CEXes, cross-border capital controls, the latency of transactions, and limited trading options. Even though arbitrage opportunities can be easily found and persist for several hours, it is still not feasible for traders to implement arbitrage strategies across CEXes. This section mainly discusses how arbitrage strategies can be implemented in DEXes overcoming constraints in CEXes and suggests further studies to consider DEXes to analyze trading behavior in financial markets.

When traders want to sell their cryptocurrencies in CEXes, they have to first transfer their assets to the platform. This may take multiple minutes to hours. After that, they can trade with their assets on CEXes.
Traders also need to pay the gas fee to the miners to realize the transfer of cryptocurrencies between the two CEXes. 
Nowadays, there are dozens of CEXes all over the world, and arbitrage opportunities may appear between any two of them.
Traders can either move their assets frequently across different CEXes for arbitrage. In this case, they have to wait a long time for cryptocurrency transactions and pay a lot of gas fees. Alternatively, they may stick to a few CEXes and only perform arbitrages within them. In this case, they may lose many arbitrage opportunities. Moreover, after depositing cryptocurrencies in CEXes, traders already lose control of their assets. Recently, one of the leading CEXes has halted cryptocurrency withdrawals from their platforms~\cite{OKEX}, indicating the risk that the CEXes operator might misappropriate traders' assets.

In DEXes, traders always (at any state of the transaction) keep their assets within their own accounts (wallets). DEXes smart contracts only swap assets between trading account (the protocol of ERC20 tokens allows DEXes smart contract accounts to remove assets from approval accounts) but not reserve traders' assets in their own accounts.
Therefore, traders can easily trade across different DEXes, even within a single transaction. They can efficiently utilize price deviations in different markets.

Another advantage of implementing arbitrage strategies in DEXes is that DEXes are not under cross-border capital control. In many CEXes, traders exchange cryptocurrencies with fiat currencies. For example, if arbitrageurs want to perform arbitrages within bitFlyer and Coinbase, they have to exchange the fiat currency of Japan and the US to ensure that their profits are not stuck in a country. In such a case, capital controls play an important role in implementing arbitrage strategies in CEXes. Capital controls do not influence trades in DEXes because all trading assets in DEXes are cryptocurrencies, which is stored in Ethereum or other blockchain systems. There is no need for traders to exchange fiat currencies immediately after cyclic arbitrage because they already earn profits in the same cryptocurrency that they own. 

Finally, DEXes enable more trading options. As we have shown in \autoref{sec:ato}, traders can perform atomic transactions to ensure the consistency of several exchanges, which is the basis of the implementation of cyclic arbitrages. Meanwhile, smart contract technology ensures positive revenue of the transaction, which limits the risk of losing money.
Moreover, other decentralized finance applications support more arbitrage possibilities. For example, flash loan applications~\cite{daian2020flash}, allow traders to borrow any amount of money (less than the amount reserved in the flash loan smart contracts) to apply arbitrage strategies if they can return the money back within the same transaction. Combined with cyclic arbitrages, traders do not need to keep any assets in their accounts to apply arbitrage transactions. They can easily use a huge amount of money to benefit themselves from price deviations, which greatly encourages more traders to participate in DEXes.
Meanwhile, if their arbitrage transactions fail or do not have enough money to pay back to flash loan contracts, the system state will be reverted to the original state and ensures the safety of the money reserved in flash loan smart contracts.

These advantages of DEXes over CEXes suggest that arbitrage is happening more often in DEXes. As a result, exchange rates in DEXes will have less arbitrage potential. This again means that regular DEX customers have to worry less that the exchange rate is far from the truth.


\subsection{Resilience to Front-running}

Despite clear benefits in implementing arbitrage strategies in DEXes, the fundamental weakness of DEXes still keeps many traders resistant to the new markets: on-chain trades are somewhat slow. The average time of generating an Ethereum block is 15 seconds. Attackers may front-run transactions: They may observe an arbitrage transaction before the generation of the block and place their own transaction with higher fees.

In \autoref{sec:fa}, we present the significant success rate of two different implementations of cyclic transactions. In general, two reasons can lead to the fail of cyclic arbitrages. The first one is a (random) change of the market state. Other transactions that are performed in advance of the cyclic transactions may change the exchange rate of the trading pair, resulting in a negative revenue. Secondly, there are front-running attacks~\cite{daian2020flash} from other arbitrageurs. Especially for those transactions interacting with public smart contracts, attackers can easily understand the arbitrage strategy of the transaction and actively create their own transactions in front of the original one to grab the benefits. In such a case, the original cyclic transaction will also fail because the front-running attackers have already balanced the market prices.

The probability that a cyclic transaction failed because of the price fluctuations should be similar with two different implementations. Therefore, the resistance to front-running determines the success rate of the two different implementations. 
Assume that the price fluctuations influence $x\%$ of transactions, then $1-\frac{\mbox{success rate}}{1-x\%}$ of cyclic transactions have been front-run by attackers. Given the huge variance between the success rate of two implementations of cyclic transactions (62\% vs. 28.4\%), our empirical analysis suggests that deploying private smart contracts can be resilient to at least 30\% more of front-running attacks than directly calling public smart contracts.

For front-running attackers, if the smart contract is not open-source, they have to replay the transaction locally to identify whether the transaction is profitable. If the smart contracts use authentication schemes such that only their own EOAs can call smart contract functions, then it is more challenging for attackers to copy the arbitrage strategy in a short time.


\iffalse

\section{Influence of Cyclic Arbitrages in Market}

\label{sec:lp}

\begin{lemma}
The market price after cyclic transactions is more balanced than the price before the cyclic transactions. In other words, there are fewer arbitrage opportunities after the cyclic transactions.
\end{lemma}

\begin{proof}
Consider a cyclic transaction through trading path $\delta_a$ through $A\rightarrow B^n\rightarrow \ldots \rightarrow B^1\rightarrow A$.

A cyclic transaction is profitable through the path if the product of exchange rates before the transaction satisfies $\frac{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}>\frac{1}{r_1^{n+1}\cdot r_2^{n+1}}$.

After the transaction, the product have to satisfy 

$\frac{(a_{n+1}-\delta_a')\cdot (b^1_1-\delta{b^1})\cdot (b^2_2-\delta_{b^2})\cdot \ldots\cdot b^n_n}{(a_1+\delta_a)\cdot (b^1_2+\delta_{b^1})\cdot (b^2_3+\delta_{b^2})\cdot\ldots\cdot (b^n_{n+1}+\delta_{b^n})}>r_1^{n+1}\cdot r_2^{n+1}$. Otherwise, there is no income for arbitrageurs from this transaction. Thus, this cyclic transaction will not be executed.

Before the cyclic transaction, for two tokens in the market, such as $A$ and $B_i$, there are two market exchange rates between them, namely $\frac{a_1}{b^1_1}\cdot \frac{b^1_2}{b^2_2}\cdot\ldots\cdot\frac{b^{i-1}_i}{b^i_i}$ and $\frac{a_{n+1}}{b^n_{n+1}}\cdot \frac{b^n_n}{b^{n-1}_n}\cdot\ldots\cdot\frac{b^{i+1}_{i+1}}{b^i_{i+1}}$. The arbitrage index of these two prices is exactly $\frac{a_{n+1}\cdot b^1_1\cdot b^2_2\cdot \ldots\cdot b^n_n}{a_1\cdot b^1_2\cdot b^2_3\cdot\ldots\cdot b^n_{n+1}}$, which is larger than $\frac{1}{r_1^{n+1}\cdot r_2^{n+1}}$.

Similarly, after the cyclic transaction, the arbitrage index of two market exchange prices between $A$ and $B_i$ is less than $\frac{1}{r_1^{n+1}\cdot r_2^{n+1}}$. Therefore, the market price is more balanced after cyclic transactions.

\end{proof}

\begin{lemma}
    If the market is efficient, liquidity providers gain more transaction fees if cyclic transactions appear during the convergence of the market prices.
\end{lemma}

\begin{proof}

Consider the exchange rate between tokens $A$ and $B$ is $\frac{a}{b} = r$ at time point $t$, and rational traders would like to move this rate to $r'$ by a transaction $T$.

Assume there is cyclic transaction $T^c$ happens at $t$ and moves the exchange rate to $r_c$. We analyze how this cyclic transaction changes the profit of liquidity providers.

If $r_c=r'$, which means that $T^c$ already moves the market price as other traders want. There is no need for an additional transaction $T$. Cyclic transaction $T^c$ does not change the profit of liquidity providers while it just substitutes of the original trade $T$.

Otherwise, $r_c\neq r'$, which means there will be another transaction $T'$ to move the market price to $r'$. Then we compare the profit of liquidity providers with $T$, and with the combination of $T^c$ and $T'$.

We assume that $T=(+\delta_{a}, -\delta_b)$, where traders would like to exchange $\delta_{a}$ of $A$ with $\delta_{b}$ of $B$ from the market. There are three scenarios according to the cyclic transaction $T^c$ and $T'$.

\begin{itemize}
    \item $T^c=(+\delta_{a}^{c}, -\delta_b^{c})$ and $T'=(-\delta_a', +\delta_b')$: 
    We can deduct that $\delta_{a}^{c}>\delta_{a}$. It turns out that $T^c$ leaves $\delta_{a}^{c}\cdot(1-r_1)$ of token $A$ as the transaction fee in the liquidity pool, which is more than what $T$ can contribute to the liquidity pool. Therefore, liquidity providers earn more transaction fees because of the cyclic transaction.
    
    \item $T^c=(-\delta_{a}^{c}, +\delta_b^{c})$ and $T'=(+\delta_a', -\delta_b')$: 
    We can deduct that $\delta_a'>\delta_a$. It turns out that $T'$ leaves $\delta_a'\cdot(1-r_1)$ of token $A$ as the transaction fee in the liquidity pool, which is more than what $T$ can contribute to the liquidity pool. Therefore, liquidity providers earn more transaction fees because of the cyclic transaction.
    
    \item $T^c=(+\delta_{a}^{c}, -\delta_b^{c})$ and $T'=(+\delta_a', -\delta_b')$: 
    The cyclic transaction  $T^c$ leaves $\delta_{a}^{c}\cdot(1-r_1)$ of token $A$ as transaction fee in the liquidity pool. Because the product of tokens' volume is a constant in Uniswap, after the cyclic transaction $T^c$, the product of tokens' volume is increased by $\delta_{a}^c\cdot(1-r_1)\cdot(b-\delta_b^c)$. Meanwhile, the exchange rates between $A$ and $B$ after $T$ and $T'$ are the same. Therefore, $T^c$ and $T'$ leave more transaction fees in the liquidity pool then $T$.
\end{itemize}
\end{proof}

\section{Arbitrageur Performance}

\begin{figure*}
    \centering
    \input{topbot_daily_revenue}
    \caption{Revenue for top 10 cyclic arbitrageurs over time.}
    \label{fig:topbots}
\end{figure*}

\autoref{fig:topbots} shows the daily arbitrage revenue of the top 10 arbitrageurs we observed with the highest total revenue. These arbitrageurs are (private) smart contracts that implement arbitrage strategies. Only creators or other authorized licensed EOAs have access to call them (an arbitrageur may use multiple EOAs to initiate arbitrage transactions). The figure suggests a dual oligopoly market from May to August where two arbitrageurs (\textcolor{blue}{0x860bd2\ldots} and \textcolor{blue}{0x693c18\ldots}) dominate the revenue of cyclic transactions. Since September, more competitors have appeared in the market. Even though \textcolor{blue}{0x860bd2\ldots} still leads in the market for most of the time, other arbitrageurs can share the revenue of the market and sometimes outperform \textcolor{blue}{0x860bd2\ldots}.

\section{Popular Trading Cycles}

\label{sec:popular}

\begin{figure*}
    \centering
    \input{top10_paths}
    \caption{The number of cyclic transactions performed on top cycles over time. }
    \label{fig:toppaths}
\end{figure*}

\autoref{fig:toppaths} demonstrates that the most popular trading cycle over time. Due to the relatively short lifespan of cryptocurrencies, most of them are only active during a certain period of time, around one month. After the active period, the exchange rates between these tokens become stable, and the market size of these tokens shrinks, resulting in less cyclic arbitrage opportunities.


\section{Block-wise Arbitrage Index}
\label{sec:blo}

\setlength{\belowcaptionskip}{0cm}

\begin{table*}[h]
    \centering
    \begin{tabular}{|c|c||c|c||c|c||c|c|}
    \hline
         token $A$ & token $B$ & token $A$ & token $B$ & token $A$ & token $B$ & token $A$ & token $B$\\
         \hline
         \hline
         YAM & yCRV& XFI & XSP & FRM & FRMX & REVV & LCX\\
         \hline
         XRT & RWS & \$BASED & sUSD & HEGIC & zHEGIC & XAMP & TOB\\
         \hline
         BADGER & WBTC  & TRB & DAI & & & &\\
         \hline
    \end{tabular}
    \caption{Tokens for computing the block-wise arbitrage index in Uniswap.}
    \label{table:arin}
\end{table*}


\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{YAM}
\caption{Block-wise arbitrage index of YAM in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{XRT}
\caption{Block-wise arbitrage index of XRT in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{BADGER.png}
\caption{Block-wise arbitrage index of BADGER in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{XFI}
\caption{Block-wise arbitrage index of XFI in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{BASED.png}
\caption{Block-wise arbitrage index of \$BASED in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{TRB}
\caption{Block-wise arbitrage index of TRB in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{FRM}
\caption{Block-wise arbitrage index of FRM in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{HEGIC}
\caption{Block-wise arbitrage index of HEGIC in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{REVV}
\caption{Block-wise arbitrage index of REVV in Uniswap.}
\end{figure*}

\begin{figure*}[hpt]
\centering
\includegraphics[width=13cm]{XAMP}
\caption{Block-wise arbitrage index of XAMP in Uniswap.}
\end{figure*}
\fi

==> review.tex <==
Review #70A
===========================================================================

Overall merit
-------------
1. Bottom 50% of submitted papers

Reviewer confidence
-------------------
3. Confident

Technical correctness
---------------------
2. Flawed but probably fixable

Paper summary
-------------
The paper studies arbitrage opportunities/behavior in a specific cryptocurrency market (Uniswap). The authors nicely explain the context of the market, describe the measurements (too succinctly). They carry on with an analysis of the Uniswap liquidity

Reasons to accept
-----------------
Interesting behavior in the context of cryptocurrencies, that suggests there might be interesting measurements to be done in the area of crypto exchanges.

Reasons to reject
-----------------
- Measurements are not validated/checked against ground truth.
- Too short/superficial description of measurements methodology.
- The measurements are not a contribution that has value for the community due to the very narrow context (UniSwap+cyclic arbitrage transactions).
- Insights focused on arbitrage opportunities in cryptocurrency markets, hence the work is out-of-scope for a conference like IMC.

Comments for author
-------------------
Abstract:
----------

The abstract clearly sets the scope of the paper, and the contributions. However, the insights being focused on arbitrage opportunities in cryptocurrency markets, makes this work rather out-of-scope for a conference like IMC. The measurement side is not a contribution on its own that has value for the community.

Introduction:
--------------

I understand that this problem of seeing such cyclic arbitrage is very interesting from the perspective of understanding cryptocurrencies and their complexity/dependencies. However, I fial to see why IMC would be the venue for this, however interesting the topic is.

At "The total cost of executing cyclic transactions is 9,520.23 ETH, only accounting for 30% of the revenue of cyclic transactions": Well that's a good fraction of the total revenue of these transactions, so I don't understand the "only" (compared to what could it be "only"?).

Cyclic arbitrage account for only 1% of all transactions: is that really so significant from a global trading volume? Please clarify/discuss.

Background:
--------------

Section 2.2: 2 typo's "executes" and "Ethereum".

Section 2.3.2: It's quite clear that because this is a new topic/area, a lot of background is necessary. While this makes the paper interesting, it also makes it clearly very "early stage" in terms of the awareness of the community, and will also make the paper as much a tutorial on DEXes as one with insight into the cyclic arbitrage. As much as I think the topic is interesting, the background section makes it clear that the area is not Internet measurements (or the SIGCOMM community), but rather economics of specific distributed systems (here cryptocurrencies).

Section 2.3.2: ERC20 contracts, Uniswap, and liquidity pools are very specific constructs that are not something generic within distributed ledgers and cryptocurrencies. While this topic is interesting, it is way too narrow on the specific choice of the UniSwap DEXes and how these work. This is in no way general enough even in terms of distributed crypto to be of interest to the SIGCOMM community. The target audience is really anyone interested in such markets, not the Internet measurements community or data communications researchers (SIGCOMM).

Overall in the background, I feel that there is way too much background necessary for the audience of IMC to understand the paper. I fear that most readers will have lost interest somewhere in Section 2, unless they want to learn about this, as I do (but that's only because I have many students interested in this, and my partner has worked on smart contracts).

Data collection:
-----------------

How extensive is this sample of the Uniswap trading pools, and of the transactions. Did you check against some ground truth?

How confident are you that your estimated/guessed failed transactions sample is correct? Do you have a ground truth to have an idea of how complete your data is overall? It does not seem like this is the case, which is something this community would need to know to trust the measurements.

Cyclic arbitrages:
-------------------

Subsection 4.1 does not tell much about the actual opportunities in terms of arbitrage, given that this is a sample of the tokens (ten popular ones, not even the most popular). The authors should first estimate the actual potential in arbitrage that exists (making optimistic assumptions and using past data), then observe how actual traders have sampled these through the actual transactions. Then, introduce the problem of the instability of the exchange rates, which will limit the opportunities or at least lead to risks in the actual return.

I don't think the authors have the story worked out quite yet, as Section 4 until 4.4 goes through rather arbitrary aspects without flowing in a natural way for the reader. (see the previous comment)

Section 4.4 is rather handwavy, in that it relies too much on Lemma 1 which discounts the whole dynamics of the system, which is likely to be very important in how traders choose to pick the opportunities most likely to lead to profit. Obviously, short cycles will suffer from less variability in the exchange rates, and look less risky than longer cycles. The authors should do a survey among traders to understand what heuristics they rely on to pick opportunities and likely limit the risks in the exchange rates. Section 4 is really not insightful, as Lemma is way too disconnected from reality to be informative.

Cost if cyclic arbitrages:
---------------------------

You claim that in 5.2 that the risk of cyclic arbitrages is negligible. You are taking a sample, possibly biased. Now, it could be that it's because arbitrageurs are smart enough to limit these risks. Just seeing the there is negligible is interesting, but asks for the reason for this.

Again some interesting observations in Section 5, but no attempt to find out why.

Impact on market:
---------------------

I'm not sure what's the point of section 6 overall. The market price balance section makes sense, so as such does not require so much space. Same for 6.2 in that it is largely irrelevant. Instead of this section, the authors would benefit from some depth in the previous section.

Discussion:
------------

As much as the discussion section is interesting for people who care about the topic, it is of little interest to the IMC community at all (even less than the results). If the authors wanted to address the community, they would focus on what measurements would be needed to answer specific questions that the IMC community could answer.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #70B
===========================================================================

Overall merit
-------------
1. Bottom 50% of submitted papers

Reviewer confidence
-------------------
2. Somewhat confident

Technical correctness
---------------------
1. Flawed, probably not fixable for IMC 2021

Paper summary
-------------
The paper presents a study of cyclic arbitrage in decentralized exchange markets. They focus on one particular market, Uniswap, gathering its full set of transactions on Etherum. Among other things, they find that cyclic arbitrage does occur.

Reasons to accept
-----------------
+ Interesting topic, will generate attention from people working in this space
+ The authors spot and quantify an interesting property of DEXs

Reasons to reject
-----------------
- There are a number of queries related to the methodology/results - these need clarification
- Some sections are inconclusive or lack robust numbers to back up statements
- There are presentation issues, which mean there is a lot of scope for improvements.

Comments for author
-------------------
The paper presents a study of cyclic arbitrage in decentralized exchange markets. They focus on one particular market, Uniswap, gathering its full set of transactions on Etherum. Among other things, they find that cyclic arbitrage does occur. The paper touches upon an interesting topic and there is a lot of scope for measurement work in this area. I think thank the authors for the work and see a lot of potential. However, I think the paper in its current form requires further work before being ready for publication. There are several parts where the methodology is unclear and requires clarification. The analysis presented also requires further work; this may be a presentation issue or, alternatively, further analysis work may be required. I have tried to be precise in listing the details of updates I think will improve the paper below:

* The introduction is long and diffuse - it could benefit from some clearer structuring. You start off with background on CEX/DEX, before talking about cyclic arbitrage. It then moves into a discussion of related work, and stating that prior research has not looked at the problem before (but this would be better suited to earlier in the intro). The following paragraphs then talk about various findings, but do so with little clear structure. I would suggest condensing this text and linking it more clearly into the overall structure of the paper. Finally, the contributions paragraph at the end would be better suited to bullet points IMHO.

* Why did you choose to only inspect Uniswap? There are quite a large number of DEX you could look at, including ones that may be in fact larger, e.g. Mdex. It would not be a huge amount of extra work to look at multiple DEXes as the analysis would be the same. At least, it would be useful to include some justification text that also touches upon how generalizable these Uniswap-centric insights might be.

* Do you only include cycles that occur on the same transaction receipt? What if an addr staggers the transfers? Surely this would also be classed as a cycle? Moreover, what fraction of overall transactions does the 285,127 cyclic transactions constitute?

* In Section 4.1, why do you only take 10 "popular" tokens? By what metric do you define "popular"? The most frequently transacted? Considering the number of tokens available to date, does this not miss a significant fraction?

* "We take the high price divided by the low price as the arbitrage index of token �� with ETH at the block" -> I was not clear why you did this. Why not take the price at a given time point, rather than diving high by low? Is this to offer the 'best case' for a trader (buy low, sell high)?

* Why does Figure 3 show the average? This is the average across the 10 popular tokens? What is the variance across these 10 tokens? Why not simply plot each one separately? It would also be useful to include more analytical text to explain the key observations from this figure.

* What is the purpose of Section 4.2? Adding some clear breadcrumb text would really improve the paper IMHO.

* "When computing the revenue of cyclic transactions in Uniswap, we only consider those that start with ETH because the majority of the proceeds of cyclic transactions are in ETH". This doesn't seem such a great reason. What do you mean by majority? This could be 51%. You then say "the exchange rate between ETH and other tokens fluctuates dramatically, which is difficult to unify" - what do you mean by unify?

* In Section 4, how many addresses were involved in these cyclic arbitrages? Was it a small set that repeatedly performed cyclic arbitrages, or a wider set that occasionally do it? Also, do you have any insights into how these opportunities are identified by traders? Is it a manual procedure or are there automated tools for spotting opportunities? What is the typical delay you observe between an opportunity arising and a trader exploiting it?

* Do the results in Section 5.1 differ from any other form of transactions? Naturally, the higher the gas, the higher the priority. Did you spot any unique trends here? When reaching the end of the section, it is not really clear what the take home message is.

* What were the defects referred to when you said "arbitrageurs have a low success rate because of the defective design of their smart contracts"?

* In Figure 14, it is still not clear why you only consider CAs that start with ETH? Also, you do not quantify what fraction this misses.

* Figure 5.2 is quite inconclusive, and raises questions that it does not really nail down. For example, you say things like "these numbers do not look perfect" and "we overestimate the number of failed transactions". Yet you do really quantify these issues. I would suggest expanding this section to quantify to what extent the analysis suffers from these issues.

* In Section 6.1, what do you mean by "cyclic arbitrages can effectively balance the price between tokens"? Could you define "balance" here? This means that the utility of a CA reduces?

* "Our result shows that the market price is always balanced after cyclic transactions, where the arbitrage index of these cycles always becomes smaller than the previous index" -> To clarify, this is always true? In every single case you observe this? If so, I would suggest making this very clear in the text.

* I was not clear on the conclusion of Section 6.2? What finding are you wishing to highlight here? The only result alluded to is the correlation coefficient, but you do not actually present any stats here. Also, you don't explicitly state what you are correlating and how you do it. Thus, it would be possible for somebody to reproduce this.

* Overall I think the paper has potential to be really strong, but I think it would benefit from revisions and further work before publication.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
